SemML: Enhancing Automata-Theoretic LTL Synthesis with Machine Learning

Synthesizing a reactive system from specifications given in linear temporal logic (LTL) is a classical problem, finding its applications in safety-critical systems design. We present our tool SemML, which won this year's LTL realizability tracks of SYNTCOMP, after years of domination by Strix. While both tools are based on the automata-theoretic approach, ours relies heavily on (i) Semantic labelling, additional information of logical nature, coming from recent LTL-to-automata translations and decorating the resulting parity game, and (ii) Machine Learning approaches turning this information into a guidance oracle for on-the-fly exploration of the parity game (whence the name SemML). Our tool fills the missing gaps of previous suggestions to use such an oracle and provides an efficeint implementation with additional algorithmic improvements. We evaluate SemML both on the entire set of SYNTCOMP as well as a synthetic data set, compare it to Strix, and analyze the advantages and limitations. As SemML solves more instances on SYNTCOMP and does so significantly faster on larger instances, this demonstrates for the first time that machine-learning-aided approaches can out-perform state-of-the-art tools in real LTL synthesis.

==> data/table_commands.tex <==
\newcommand{\StrixRealSyntcompZero}{522}
\newcommand{\StrixUnrealSyntcompZero}{421}
\newcommand{\SemmlARealSyntcompZero}{532}
\newcommand{\SemmlAUnrealSyntcompZero}{432}
\newcommand{\SemmlRealSyntcompZero}{534}
\newcommand{\SemmlUnrealSyntcompZero}{431}
\newcommand{\trivialSyntcompZero}{0}
\newcommand{\nontrivialSyntcompZero}{1056}
\newcommand{\trivialStrixSemmlASyntcompZero}{0}
\newcommand{\unknownStrixSemmlASyntcompZero}{59}
\newcommand{\StrixSemmlASyntcompZeroAllT}{0.15}
\newcommand{\StrixSemmlASyntcompZeroAllM}{910}
\newcommand{\StrixSemmlASyntcompZeroAllK}{33}
\newcommand{\StrixSemmlASyntcompZeroAllL}{54}
\newcommand{\StrixSemmlASyntcompZeroAllScore}{\StrixSemmlASyntcompZeroAllT[\StrixSemmlASyntcompZeroAllM+\StrixSemmlASyntcompZeroAllK/\StrixSemmlASyntcompZeroAllL]}
\newcommand{\StrixSemmlASyntcompZeroRealT}{0.13}
\newcommand{\StrixSemmlASyntcompZeroRealM}{508}
\newcommand{\StrixSemmlASyntcompZeroRealK}{14}
\newcommand{\StrixSemmlASyntcompZeroRealL}{24}
\newcommand{\StrixSemmlASyntcompZeroRealScore}{\StrixSemmlASyntcompZeroRealT[\StrixSemmlASyntcompZeroRealM+\StrixSemmlASyntcompZeroRealK/\StrixSemmlASyntcompZeroRealL]}
\newcommand{\StrixSemmlASyntcompZeroUnrealT}{0.16}
\newcommand{\StrixSemmlASyntcompZeroUnrealM}{402}
\newcommand{\StrixSemmlASyntcompZeroUnrealK}{19}
\newcommand{\StrixSemmlASyntcompZeroUnrealL}{30}
\newcommand{\StrixSemmlASyntcompZeroUnrealScore}{\StrixSemmlASyntcompZeroUnrealT[\StrixSemmlASyntcompZeroUnrealM+\StrixSemmlASyntcompZeroUnrealK/\StrixSemmlASyntcompZeroUnrealL]}
\newcommand{\trivialStrixSemmlSyntcompZero}{0}
\newcommand{\unknownStrixSemmlSyntcompZero}{64}
\newcommand{\StrixSemmlSyntcompZeroAllT}{0.09}
\newcommand{\StrixSemmlSyntcompZeroAllM}{916}
\newcommand{\StrixSemmlSyntcompZeroAllK}{27}
\newcommand{\StrixSemmlSyntcompZeroAllL}{49}
\newcommand{\StrixSemmlSyntcompZeroAllScore}{\StrixSemmlSyntcompZeroAllT[\StrixSemmlSyntcompZeroAllM+\StrixSemmlSyntcompZeroAllK/\StrixSemmlSyntcompZeroAllL]}
\newcommand{\StrixSemmlSyntcompZeroRealT}{0.08}
\newcommand{\StrixSemmlSyntcompZeroRealM}{510}
\newcommand{\StrixSemmlSyntcompZeroRealK}{12}
\newcommand{\StrixSemmlSyntcompZeroRealL}{24}
\newcommand{\StrixSemmlSyntcompZeroRealScore}{\StrixSemmlSyntcompZeroRealT[\StrixSemmlSyntcompZeroRealM+\StrixSemmlSyntcompZeroRealK/\StrixSemmlSyntcompZeroRealL]}
\newcommand{\StrixSemmlSyntcompZeroUnrealT}{0.1}
\newcommand{\StrixSemmlSyntcompZeroUnrealM}{406}
\newcommand{\StrixSemmlSyntcompZeroUnrealK}{15}
\newcommand{\StrixSemmlSyntcompZeroUnrealL}{25}
\newcommand{\StrixSemmlSyntcompZeroUnrealScore}{\StrixSemmlSyntcompZeroUnrealT[\StrixSemmlSyntcompZeroUnrealM+\StrixSemmlSyntcompZeroUnrealK/\StrixSemmlSyntcompZeroUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcompZero}{0}
\newcommand{\unknownSemmlASemmlSyntcompZero}{82}
\newcommand{\SemmlASemmlSyntcompZeroAllT}{0.61}
\newcommand{\SemmlASemmlSyntcompZeroAllM}{955}
\newcommand{\SemmlASemmlSyntcompZeroAllK}{9}
\newcommand{\SemmlASemmlSyntcompZeroAllL}{10}
\newcommand{\SemmlASemmlSyntcompZeroAllScore}{\SemmlASemmlSyntcompZeroAllT[\SemmlASemmlSyntcompZeroAllM+\SemmlASemmlSyntcompZeroAllK/\SemmlASemmlSyntcompZeroAllL]}
\newcommand{\SemmlASemmlSyntcompZeroRealT}{0.63}
\newcommand{\SemmlASemmlSyntcompZeroRealM}{531}
\newcommand{\SemmlASemmlSyntcompZeroRealK}{1}
\newcommand{\SemmlASemmlSyntcompZeroRealL}{3}
\newcommand{\SemmlASemmlSyntcompZeroRealScore}{\SemmlASemmlSyntcompZeroRealT[\SemmlASemmlSyntcompZeroRealM+\SemmlASemmlSyntcompZeroRealK/\SemmlASemmlSyntcompZeroRealL]}
\newcommand{\SemmlASemmlSyntcompZeroUnrealT}{0.59}
\newcommand{\SemmlASemmlSyntcompZeroUnrealM}{424}
\newcommand{\SemmlASemmlSyntcompZeroUnrealK}{8}
\newcommand{\SemmlASemmlSyntcompZeroUnrealL}{7}
\newcommand{\SemmlASemmlSyntcompZeroUnrealScore}{\SemmlASemmlSyntcompZeroUnrealT[\SemmlASemmlSyntcompZeroUnrealM+\SemmlASemmlSyntcompZeroUnrealK/\SemmlASemmlSyntcompZeroUnrealL]}
\newcommand{\StrixRealSyntheticZero}{8}
\newcommand{\StrixUnrealSyntheticZero}{22}
\newcommand{\SemmlARealSyntheticZero}{27}
\newcommand{\SemmlAUnrealSyntheticZero}{40}
\newcommand{\SemmlRealSyntheticZero}{35}
\newcommand{\SemmlUnrealSyntheticZero}{48}
\newcommand{\trivialSyntheticZero}{0}
\newcommand{\nontrivialSyntheticZero}{200}
\newcommand{\trivialStrixSemmlASyntheticZero}{0}
\newcommand{\unknownStrixSemmlASyntheticZero}{133}
\newcommand{\StrixSemmlASyntheticZeroAllT}{9.1}
\newcommand{\StrixSemmlASyntheticZeroAllM}{30}
\newcommand{\StrixSemmlASyntheticZeroAllK}{0}
\newcommand{\StrixSemmlASyntheticZeroAllL}{37}
\newcommand{\StrixSemmlASyntheticZeroAllScore}{\StrixSemmlASyntheticZeroAllT[\StrixSemmlASyntheticZeroAllM+\StrixSemmlASyntheticZeroAllK/\StrixSemmlASyntheticZeroAllL]}
\newcommand{\StrixSemmlASyntheticZeroRealT}{10.44}
\newcommand{\StrixSemmlASyntheticZeroRealM}{8}
\newcommand{\StrixSemmlASyntheticZeroRealK}{0}
\newcommand{\StrixSemmlASyntheticZeroRealL}{19}
\newcommand{\StrixSemmlASyntheticZeroRealScore}{\StrixSemmlASyntheticZeroRealT[\StrixSemmlASyntheticZeroRealM+\StrixSemmlASyntheticZeroRealK/\StrixSemmlASyntheticZeroRealL]}
\newcommand{\StrixSemmlASyntheticZeroUnrealT}{8.66}
\newcommand{\StrixSemmlASyntheticZeroUnrealM}{22}
\newcommand{\StrixSemmlASyntheticZeroUnrealK}{0}
\newcommand{\StrixSemmlASyntheticZeroUnrealL}{18}
\newcommand{\StrixSemmlASyntheticZeroUnrealScore}{\StrixSemmlASyntheticZeroUnrealT[\StrixSemmlASyntheticZeroUnrealM+\StrixSemmlASyntheticZeroUnrealK/\StrixSemmlASyntheticZeroUnrealL]}
\newcommand{\trivialStrixSemmlSyntheticZero}{0}
\newcommand{\unknownStrixSemmlSyntheticZero}{117}
\newcommand{\StrixSemmlSyntheticZeroAllT}{8.56}
\newcommand{\StrixSemmlSyntheticZeroAllM}{30}
\newcommand{\StrixSemmlSyntheticZeroAllK}{0}
\newcommand{\StrixSemmlSyntheticZeroAllL}{53}
\newcommand{\StrixSemmlSyntheticZeroAllScore}{\StrixSemmlSyntheticZeroAllT[\StrixSemmlSyntheticZeroAllM+\StrixSemmlSyntheticZeroAllK/\StrixSemmlSyntheticZeroAllL]}
\newcommand{\StrixSemmlSyntheticZeroRealT}{13.07}
\newcommand{\StrixSemmlSyntheticZeroRealM}{8}
\newcommand{\StrixSemmlSyntheticZeroRealK}{0}
\newcommand{\StrixSemmlSyntheticZeroRealL}{27}
\newcommand{\StrixSemmlSyntheticZeroRealScore}{\StrixSemmlSyntheticZeroRealT[\StrixSemmlSyntheticZeroRealM+\StrixSemmlSyntheticZeroRealK/\StrixSemmlSyntheticZeroRealL]}
\newcommand{\StrixSemmlSyntheticZeroUnrealT}{7.33}
\newcommand{\StrixSemmlSyntheticZeroUnrealM}{22}
\newcommand{\StrixSemmlSyntheticZeroUnrealK}{0}
\newcommand{\StrixSemmlSyntheticZeroUnrealL}{26}
\newcommand{\StrixSemmlSyntheticZeroUnrealScore}{\StrixSemmlSyntheticZeroUnrealT[\StrixSemmlSyntheticZeroUnrealM+\StrixSemmlSyntheticZeroUnrealK/\StrixSemmlSyntheticZeroUnrealL]}
\newcommand{\trivialSemmlASemmlSyntheticZero}{0}
\newcommand{\unknownSemmlASemmlSyntheticZero}{113}
\newcommand{\SemmlASemmlSyntheticZeroAllT}{1.36}
\newcommand{\SemmlASemmlSyntheticZeroAllM}{63}
\newcommand{\SemmlASemmlSyntheticZeroAllK}{4}
\newcommand{\SemmlASemmlSyntheticZeroAllL}{20}
\newcommand{\SemmlASemmlSyntheticZeroAllScore}{\SemmlASemmlSyntheticZeroAllT[\SemmlASemmlSyntheticZeroAllM+\SemmlASemmlSyntheticZeroAllK/\SemmlASemmlSyntheticZeroAllL]}
\newcommand{\SemmlASemmlSyntheticZeroRealT}{1.67}
\newcommand{\SemmlASemmlSyntheticZeroRealM}{25}
\newcommand{\SemmlASemmlSyntheticZeroRealK}{2}
\newcommand{\SemmlASemmlSyntheticZeroRealL}{10}
\newcommand{\SemmlASemmlSyntheticZeroRealScore}{\SemmlASemmlSyntheticZeroRealT[\SemmlASemmlSyntheticZeroRealM+\SemmlASemmlSyntheticZeroRealK/\SemmlASemmlSyntheticZeroRealL]}
\newcommand{\SemmlASemmlSyntheticZeroUnrealT}{1.19}
\newcommand{\SemmlASemmlSyntheticZeroUnrealM}{38}
\newcommand{\SemmlASemmlSyntheticZeroUnrealK}{2}
\newcommand{\SemmlASemmlSyntheticZeroUnrealL}{10}
\newcommand{\SemmlASemmlSyntheticZeroUnrealScore}{\SemmlASemmlSyntheticZeroUnrealT[\SemmlASemmlSyntheticZeroUnrealM+\SemmlASemmlSyntheticZeroUnrealK/\SemmlASemmlSyntheticZeroUnrealL]}
\newcommand{\StrixRealSyntcomptfZero}{550}
\newcommand{\StrixUnrealSyntcomptfZero}{428}
\newcommand{\SemmlARealSyntcomptfZero}{560}
\newcommand{\SemmlAUnrealSyntcomptfZero}{439}
\newcommand{\SemmlRealSyntcomptfZero}{562}
\newcommand{\SemmlUnrealSyntcomptfZero}{438}
\newcommand{\trivialSyntcomptfZero}{0}
\newcommand{\nontrivialSyntcomptfZero}{1111}
\newcommand{\trivialStrixSemmlASyntcomptfZero}{0}
\newcommand{\unknownStrixSemmlASyntcomptfZero}{79}
\newcommand{\StrixSemmlASyntcomptfZeroAllT}{0.15}
\newcommand{\StrixSemmlASyntcomptfZeroAllM}{945}
\newcommand{\StrixSemmlASyntcomptfZeroAllK}{33}
\newcommand{\StrixSemmlASyntcomptfZeroAllL}{54}
\newcommand{\StrixSemmlASyntcomptfZeroAllScore}{\StrixSemmlASyntcomptfZeroAllT[\StrixSemmlASyntcomptfZeroAllM+\StrixSemmlASyntcomptfZeroAllK/\StrixSemmlASyntcomptfZeroAllL]}
\newcommand{\StrixSemmlASyntcomptfZeroRealT}{0.15}
\newcommand{\StrixSemmlASyntcomptfZeroRealM}{536}
\newcommand{\StrixSemmlASyntcomptfZeroRealK}{14}
\newcommand{\StrixSemmlASyntcomptfZeroRealL}{24}
\newcommand{\StrixSemmlASyntcomptfZeroRealScore}{\StrixSemmlASyntcomptfZeroRealT[\StrixSemmlASyntcomptfZeroRealM+\StrixSemmlASyntcomptfZeroRealK/\StrixSemmlASyntcomptfZeroRealL]}
\newcommand{\StrixSemmlASyntcomptfZeroUnrealT}{0.17}
\newcommand{\StrixSemmlASyntcomptfZeroUnrealM}{409}
\newcommand{\StrixSemmlASyntcomptfZeroUnrealK}{19}
\newcommand{\StrixSemmlASyntcomptfZeroUnrealL}{30}
\newcommand{\StrixSemmlASyntcomptfZeroUnrealScore}{\StrixSemmlASyntcomptfZeroUnrealT[\StrixSemmlASyntcomptfZeroUnrealM+\StrixSemmlASyntcomptfZeroUnrealK/\StrixSemmlASyntcomptfZeroUnrealL]}
\newcommand{\trivialStrixSemmlSyntcomptfZero}{0}
\newcommand{\unknownStrixSemmlSyntcomptfZero}{84}
\newcommand{\StrixSemmlSyntcomptfZeroAllT}{0.09}
\newcommand{\StrixSemmlSyntcomptfZeroAllM}{951}
\newcommand{\StrixSemmlSyntcomptfZeroAllK}{27}
\newcommand{\StrixSemmlSyntcomptfZeroAllL}{49}
\newcommand{\StrixSemmlSyntcomptfZeroAllScore}{\StrixSemmlSyntcomptfZeroAllT[\StrixSemmlSyntcomptfZeroAllM+\StrixSemmlSyntcomptfZeroAllK/\StrixSemmlSyntcomptfZeroAllL]}
\newcommand{\StrixSemmlSyntcomptfZeroRealT}{0.09}
\newcommand{\StrixSemmlSyntcomptfZeroRealM}{538}
\newcommand{\StrixSemmlSyntcomptfZeroRealK}{12}
\newcommand{\StrixSemmlSyntcomptfZeroRealL}{24}
\newcommand{\StrixSemmlSyntcomptfZeroRealScore}{\StrixSemmlSyntcomptfZeroRealT[\StrixSemmlSyntcomptfZeroRealM+\StrixSemmlSyntcomptfZeroRealK/\StrixSemmlSyntcomptfZeroRealL]}
\newcommand{\StrixSemmlSyntcomptfZeroUnrealT}{0.1}
\newcommand{\StrixSemmlSyntcomptfZeroUnrealM}{413}
\newcommand{\StrixSemmlSyntcomptfZeroUnrealK}{15}
\newcommand{\StrixSemmlSyntcomptfZeroUnrealL}{25}
\newcommand{\StrixSemmlSyntcomptfZeroUnrealScore}{\StrixSemmlSyntcomptfZeroUnrealT[\StrixSemmlSyntcomptfZeroUnrealM+\StrixSemmlSyntcomptfZeroUnrealK/\StrixSemmlSyntcomptfZeroUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcomptfZero}{0}
\newcommand{\unknownSemmlASemmlSyntcomptfZero}{102}
\newcommand{\SemmlASemmlSyntcomptfZeroAllT}{0.61}
\newcommand{\SemmlASemmlSyntcomptfZeroAllM}{990}
\newcommand{\SemmlASemmlSyntcomptfZeroAllK}{9}
\newcommand{\SemmlASemmlSyntcomptfZeroAllL}{10}
\newcommand{\SemmlASemmlSyntcomptfZeroAllScore}{\SemmlASemmlSyntcomptfZeroAllT[\SemmlASemmlSyntcomptfZeroAllM+\SemmlASemmlSyntcomptfZeroAllK/\SemmlASemmlSyntcomptfZeroAllL]}
\newcommand{\SemmlASemmlSyntcomptfZeroRealT}{0.64}
\newcommand{\SemmlASemmlSyntcomptfZeroRealM}{559}
\newcommand{\SemmlASemmlSyntcomptfZeroRealK}{1}
\newcommand{\SemmlASemmlSyntcomptfZeroRealL}{3}
\newcommand{\SemmlASemmlSyntcomptfZeroRealScore}{\SemmlASemmlSyntcomptfZeroRealT[\SemmlASemmlSyntcomptfZeroRealM+\SemmlASemmlSyntcomptfZeroRealK/\SemmlASemmlSyntcomptfZeroRealL]}
\newcommand{\SemmlASemmlSyntcomptfZeroUnrealT}{0.59}
\newcommand{\SemmlASemmlSyntcomptfZeroUnrealM}{431}
\newcommand{\SemmlASemmlSyntcomptfZeroUnrealK}{8}
\newcommand{\SemmlASemmlSyntcomptfZeroUnrealL}{7}
\newcommand{\SemmlASemmlSyntcomptfZeroUnrealScore}{\SemmlASemmlSyntcomptfZeroUnrealT[\SemmlASemmlSyntcomptfZeroUnrealM+\SemmlASemmlSyntcomptfZeroUnrealK/\SemmlASemmlSyntcomptfZeroUnrealL]}
\newcommand{\StrixRealSyntcompOne}{522}
\newcommand{\StrixUnrealSyntcompOne}{421}
\newcommand{\SemmlARealSyntcompOne}{532}
\newcommand{\SemmlAUnrealSyntcompOne}{432}
\newcommand{\SemmlRealSyntcompOne}{534}
\newcommand{\SemmlUnrealSyntcompOne}{431}
\newcommand{\trivialSyntcompOne}{0}
\newcommand{\nontrivialSyntcompOne}{1056}
\newcommand{\trivialStrixSemmlASyntcompOne}{606}
\newcommand{\unknownStrixSemmlASyntcompOne}{59}
\newcommand{\StrixSemmlASyntcompOneAllT}{0.69}
\newcommand{\StrixSemmlASyntcompOneAllM}{304}
\newcommand{\StrixSemmlASyntcompOneAllK}{33}
\newcommand{\StrixSemmlASyntcompOneAllL}{54}
\newcommand{\StrixSemmlASyntcompOneAllScore}{\StrixSemmlASyntcompOneAllT[\StrixSemmlASyntcompOneAllM+\StrixSemmlASyntcompOneAllK/\StrixSemmlASyntcompOneAllL]}
\newcommand{\StrixSemmlASyntcompOneRealT}{0.81}
\newcommand{\StrixSemmlASyntcompOneRealM}{165}
\newcommand{\StrixSemmlASyntcompOneRealK}{14}
\newcommand{\StrixSemmlASyntcompOneRealL}{24}
\newcommand{\StrixSemmlASyntcompOneRealScore}{\StrixSemmlASyntcompOneRealT[\StrixSemmlASyntcompOneRealM+\StrixSemmlASyntcompOneRealK/\StrixSemmlASyntcompOneRealL]}
\newcommand{\StrixSemmlASyntcompOneUnrealT}{0.57}
\newcommand{\StrixSemmlASyntcompOneUnrealM}{139}
\newcommand{\StrixSemmlASyntcompOneUnrealK}{19}
\newcommand{\StrixSemmlASyntcompOneUnrealL}{30}
\newcommand{\StrixSemmlASyntcompOneUnrealScore}{\StrixSemmlASyntcompOneUnrealT[\StrixSemmlASyntcompOneUnrealM+\StrixSemmlASyntcompOneUnrealK/\StrixSemmlASyntcompOneUnrealL]}
\newcommand{\trivialStrixSemmlSyntcompOne}{0}
\newcommand{\unknownStrixSemmlSyntcompOne}{64}
\newcommand{\StrixSemmlSyntcompOneAllT}{0.09}
\newcommand{\StrixSemmlSyntcompOneAllM}{916}
\newcommand{\StrixSemmlSyntcompOneAllK}{27}
\newcommand{\StrixSemmlSyntcompOneAllL}{49}
\newcommand{\StrixSemmlSyntcompOneAllScore}{\StrixSemmlSyntcompOneAllT[\StrixSemmlSyntcompOneAllM+\StrixSemmlSyntcompOneAllK/\StrixSemmlSyntcompOneAllL]}
\newcommand{\StrixSemmlSyntcompOneRealT}{0.08}
\newcommand{\StrixSemmlSyntcompOneRealM}{510}
\newcommand{\StrixSemmlSyntcompOneRealK}{12}
\newcommand{\StrixSemmlSyntcompOneRealL}{24}
\newcommand{\StrixSemmlSyntcompOneRealScore}{\StrixSemmlSyntcompOneRealT[\StrixSemmlSyntcompOneRealM+\StrixSemmlSyntcompOneRealK/\StrixSemmlSyntcompOneRealL]}
\newcommand{\StrixSemmlSyntcompOneUnrealT}{0.1}
\newcommand{\StrixSemmlSyntcompOneUnrealM}{406}
\newcommand{\StrixSemmlSyntcompOneUnrealK}{15}
\newcommand{\StrixSemmlSyntcompOneUnrealL}{25}
\newcommand{\StrixSemmlSyntcompOneUnrealScore}{\StrixSemmlSyntcompOneUnrealT[\StrixSemmlSyntcompOneUnrealM+\StrixSemmlSyntcompOneUnrealK/\StrixSemmlSyntcompOneUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcompOne}{0}
\newcommand{\unknownSemmlASemmlSyntcompOne}{82}
\newcommand{\SemmlASemmlSyntcompOneAllT}{0.61}
\newcommand{\SemmlASemmlSyntcompOneAllM}{955}
\newcommand{\SemmlASemmlSyntcompOneAllK}{9}
\newcommand{\SemmlASemmlSyntcompOneAllL}{10}
\newcommand{\SemmlASemmlSyntcompOneAllScore}{\SemmlASemmlSyntcompOneAllT[\SemmlASemmlSyntcompOneAllM+\SemmlASemmlSyntcompOneAllK/\SemmlASemmlSyntcompOneAllL]}
\newcommand{\SemmlASemmlSyntcompOneRealT}{0.63}
\newcommand{\SemmlASemmlSyntcompOneRealM}{531}
\newcommand{\SemmlASemmlSyntcompOneRealK}{1}
\newcommand{\SemmlASemmlSyntcompOneRealL}{3}
\newcommand{\SemmlASemmlSyntcompOneRealScore}{\SemmlASemmlSyntcompOneRealT[\SemmlASemmlSyntcompOneRealM+\SemmlASemmlSyntcompOneRealK/\SemmlASemmlSyntcompOneRealL]}
\newcommand{\SemmlASemmlSyntcompOneUnrealT}{0.59}
\newcommand{\SemmlASemmlSyntcompOneUnrealM}{424}
\newcommand{\SemmlASemmlSyntcompOneUnrealK}{8}
\newcommand{\SemmlASemmlSyntcompOneUnrealL}{7}
\newcommand{\SemmlASemmlSyntcompOneUnrealScore}{\SemmlASemmlSyntcompOneUnrealT[\SemmlASemmlSyntcompOneUnrealM+\SemmlASemmlSyntcompOneUnrealK/\SemmlASemmlSyntcompOneUnrealL]}
\newcommand{\StrixRealSyntheticOne}{8}
\newcommand{\StrixUnrealSyntheticOne}{22}
\newcommand{\SemmlARealSyntheticOne}{27}
\newcommand{\SemmlAUnrealSyntheticOne}{40}
\newcommand{\SemmlRealSyntheticOne}{35}
\newcommand{\SemmlUnrealSyntheticOne}{48}
\newcommand{\trivialSyntheticOne}{0}
\newcommand{\nontrivialSyntheticOne}{200}
\newcommand{\trivialStrixSemmlASyntheticOne}{0}
\newcommand{\unknownStrixSemmlASyntheticOne}{133}
\newcommand{\StrixSemmlASyntheticOneAllT}{9.1}
\newcommand{\StrixSemmlASyntheticOneAllM}{30}
\newcommand{\StrixSemmlASyntheticOneAllK}{0}
\newcommand{\StrixSemmlASyntheticOneAllL}{37}
\newcommand{\StrixSemmlASyntheticOneAllScore}{\StrixSemmlASyntheticOneAllT[\StrixSemmlASyntheticOneAllM+\StrixSemmlASyntheticOneAllK/\StrixSemmlASyntheticOneAllL]}
\newcommand{\StrixSemmlASyntheticOneRealT}{10.44}
\newcommand{\StrixSemmlASyntheticOneRealM}{8}
\newcommand{\StrixSemmlASyntheticOneRealK}{0}
\newcommand{\StrixSemmlASyntheticOneRealL}{19}
\newcommand{\StrixSemmlASyntheticOneRealScore}{\StrixSemmlASyntheticOneRealT[\StrixSemmlASyntheticOneRealM+\StrixSemmlASyntheticOneRealK/\StrixSemmlASyntheticOneRealL]}
\newcommand{\StrixSemmlASyntheticOneUnrealT}{8.66}
\newcommand{\StrixSemmlASyntheticOneUnrealM}{22}
\newcommand{\StrixSemmlASyntheticOneUnrealK}{0}
\newcommand{\StrixSemmlASyntheticOneUnrealL}{18}
\newcommand{\StrixSemmlASyntheticOneUnrealScore}{\StrixSemmlASyntheticOneUnrealT[\StrixSemmlASyntheticOneUnrealM+\StrixSemmlASyntheticOneUnrealK/\StrixSemmlASyntheticOneUnrealL]}
\newcommand{\trivialStrixSemmlSyntheticOne}{0}
\newcommand{\unknownStrixSemmlSyntheticOne}{117}
\newcommand{\StrixSemmlSyntheticOneAllT}{8.56}
\newcommand{\StrixSemmlSyntheticOneAllM}{30}
\newcommand{\StrixSemmlSyntheticOneAllK}{0}
\newcommand{\StrixSemmlSyntheticOneAllL}{53}
\newcommand{\StrixSemmlSyntheticOneAllScore}{\StrixSemmlSyntheticOneAllT[\StrixSemmlSyntheticOneAllM+\StrixSemmlSyntheticOneAllK/\StrixSemmlSyntheticOneAllL]}
\newcommand{\StrixSemmlSyntheticOneRealT}{13.07}
\newcommand{\StrixSemmlSyntheticOneRealM}{8}
\newcommand{\StrixSemmlSyntheticOneRealK}{0}
\newcommand{\StrixSemmlSyntheticOneRealL}{27}
\newcommand{\StrixSemmlSyntheticOneRealScore}{\StrixSemmlSyntheticOneRealT[\StrixSemmlSyntheticOneRealM+\StrixSemmlSyntheticOneRealK/\StrixSemmlSyntheticOneRealL]}
\newcommand{\StrixSemmlSyntheticOneUnrealT}{7.33}
\newcommand{\StrixSemmlSyntheticOneUnrealM}{22}
\newcommand{\StrixSemmlSyntheticOneUnrealK}{0}
\newcommand{\StrixSemmlSyntheticOneUnrealL}{26}
\newcommand{\StrixSemmlSyntheticOneUnrealScore}{\StrixSemmlSyntheticOneUnrealT[\StrixSemmlSyntheticOneUnrealM+\StrixSemmlSyntheticOneUnrealK/\StrixSemmlSyntheticOneUnrealL]}
\newcommand{\trivialSemmlASemmlSyntheticOne}{0}
\newcommand{\unknownSemmlASemmlSyntheticOne}{113}
\newcommand{\SemmlASemmlSyntheticOneAllT}{1.36}
\newcommand{\SemmlASemmlSyntheticOneAllM}{63}
\newcommand{\SemmlASemmlSyntheticOneAllK}{4}
\newcommand{\SemmlASemmlSyntheticOneAllL}{20}
\newcommand{\SemmlASemmlSyntheticOneAllScore}{\SemmlASemmlSyntheticOneAllT[\SemmlASemmlSyntheticOneAllM+\SemmlASemmlSyntheticOneAllK/\SemmlASemmlSyntheticOneAllL]}
\newcommand{\SemmlASemmlSyntheticOneRealT}{1.67}
\newcommand{\SemmlASemmlSyntheticOneRealM}{25}
\newcommand{\SemmlASemmlSyntheticOneRealK}{2}
\newcommand{\SemmlASemmlSyntheticOneRealL}{10}
\newcommand{\SemmlASemmlSyntheticOneRealScore}{\SemmlASemmlSyntheticOneRealT[\SemmlASemmlSyntheticOneRealM+\SemmlASemmlSyntheticOneRealK/\SemmlASemmlSyntheticOneRealL]}
\newcommand{\SemmlASemmlSyntheticOneUnrealT}{1.19}
\newcommand{\SemmlASemmlSyntheticOneUnrealM}{38}
\newcommand{\SemmlASemmlSyntheticOneUnrealK}{2}
\newcommand{\SemmlASemmlSyntheticOneUnrealL}{10}
\newcommand{\SemmlASemmlSyntheticOneUnrealScore}{\SemmlASemmlSyntheticOneUnrealT[\SemmlASemmlSyntheticOneUnrealM+\SemmlASemmlSyntheticOneUnrealK/\SemmlASemmlSyntheticOneUnrealL]}
\newcommand{\StrixRealSyntcomptfOne}{550}
\newcommand{\StrixUnrealSyntcomptfOne}{428}
\newcommand{\SemmlARealSyntcomptfOne}{560}
\newcommand{\SemmlAUnrealSyntcomptfOne}{439}
\newcommand{\SemmlRealSyntcomptfOne}{562}
\newcommand{\SemmlUnrealSyntcomptfOne}{438}
\newcommand{\trivialSyntcomptfOne}{0}
\newcommand{\nontrivialSyntcomptfOne}{1111}
\newcommand{\trivialStrixSemmlASyntcomptfOne}{611}
\newcommand{\unknownStrixSemmlASyntcomptfOne}{79}
\newcommand{\StrixSemmlASyntcomptfOneAllT}{0.71}
\newcommand{\StrixSemmlASyntcomptfOneAllM}{334}
\newcommand{\StrixSemmlASyntcomptfOneAllK}{33}
\newcommand{\StrixSemmlASyntcomptfOneAllL}{54}
\newcommand{\StrixSemmlASyntcomptfOneAllScore}{\StrixSemmlASyntcomptfOneAllT[\StrixSemmlASyntcomptfOneAllM+\StrixSemmlASyntcomptfOneAllK/\StrixSemmlASyntcomptfOneAllL]}
\newcommand{\StrixSemmlASyntcomptfOneRealT}{0.83}
\newcommand{\StrixSemmlASyntcomptfOneRealM}{188}
\newcommand{\StrixSemmlASyntcomptfOneRealK}{14}
\newcommand{\StrixSemmlASyntcomptfOneRealL}{24}
\newcommand{\StrixSemmlASyntcomptfOneRealScore}{\StrixSemmlASyntcomptfOneRealT[\StrixSemmlASyntcomptfOneRealM+\StrixSemmlASyntcomptfOneRealK/\StrixSemmlASyntcomptfOneRealL]}
\newcommand{\StrixSemmlASyntcomptfOneUnrealT}{0.58}
\newcommand{\StrixSemmlASyntcomptfOneUnrealM}{146}
\newcommand{\StrixSemmlASyntcomptfOneUnrealK}{19}
\newcommand{\StrixSemmlASyntcomptfOneUnrealL}{30}
\newcommand{\StrixSemmlASyntcomptfOneUnrealScore}{\StrixSemmlASyntcomptfOneUnrealT[\StrixSemmlASyntcomptfOneUnrealM+\StrixSemmlASyntcomptfOneUnrealK/\StrixSemmlASyntcomptfOneUnrealL]}
\newcommand{\trivialStrixSemmlSyntcomptfOne}{0}
\newcommand{\unknownStrixSemmlSyntcomptfOne}{84}
\newcommand{\StrixSemmlSyntcomptfOneAllT}{0.09}
\newcommand{\StrixSemmlSyntcomptfOneAllM}{951}
\newcommand{\StrixSemmlSyntcomptfOneAllK}{27}
\newcommand{\StrixSemmlSyntcomptfOneAllL}{49}
\newcommand{\StrixSemmlSyntcomptfOneAllScore}{\StrixSemmlSyntcomptfOneAllT[\StrixSemmlSyntcomptfOneAllM+\StrixSemmlSyntcomptfOneAllK/\StrixSemmlSyntcomptfOneAllL]}
\newcommand{\StrixSemmlSyntcomptfOneRealT}{0.09}
\newcommand{\StrixSemmlSyntcomptfOneRealM}{538}
\newcommand{\StrixSemmlSyntcomptfOneRealK}{12}
\newcommand{\StrixSemmlSyntcomptfOneRealL}{24}
\newcommand{\StrixSemmlSyntcomptfOneRealScore}{\StrixSemmlSyntcomptfOneRealT[\StrixSemmlSyntcomptfOneRealM+\StrixSemmlSyntcomptfOneRealK/\StrixSemmlSyntcomptfOneRealL]}
\newcommand{\StrixSemmlSyntcomptfOneUnrealT}{0.1}
\newcommand{\StrixSemmlSyntcomptfOneUnrealM}{413}
\newcommand{\StrixSemmlSyntcomptfOneUnrealK}{15}
\newcommand{\StrixSemmlSyntcomptfOneUnrealL}{25}
\newcommand{\StrixSemmlSyntcomptfOneUnrealScore}{\StrixSemmlSyntcomptfOneUnrealT[\StrixSemmlSyntcomptfOneUnrealM+\StrixSemmlSyntcomptfOneUnrealK/\StrixSemmlSyntcomptfOneUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcomptfOne}{0}
\newcommand{\unknownSemmlASemmlSyntcomptfOne}{102}
\newcommand{\SemmlASemmlSyntcomptfOneAllT}{0.61}
\newcommand{\SemmlASemmlSyntcomptfOneAllM}{990}
\newcommand{\SemmlASemmlSyntcomptfOneAllK}{9}
\newcommand{\SemmlASemmlSyntcomptfOneAllL}{10}
\newcommand{\SemmlASemmlSyntcomptfOneAllScore}{\SemmlASemmlSyntcomptfOneAllT[\SemmlASemmlSyntcomptfOneAllM+\SemmlASemmlSyntcomptfOneAllK/\SemmlASemmlSyntcomptfOneAllL]}
\newcommand{\SemmlASemmlSyntcomptfOneRealT}{0.64}
\newcommand{\SemmlASemmlSyntcomptfOneRealM}{559}
\newcommand{\SemmlASemmlSyntcomptfOneRealK}{1}
\newcommand{\SemmlASemmlSyntcomptfOneRealL}{3}
\newcommand{\SemmlASemmlSyntcomptfOneRealScore}{\SemmlASemmlSyntcomptfOneRealT[\SemmlASemmlSyntcomptfOneRealM+\SemmlASemmlSyntcomptfOneRealK/\SemmlASemmlSyntcomptfOneRealL]}
\newcommand{\SemmlASemmlSyntcomptfOneUnrealT}{0.59}
\newcommand{\SemmlASemmlSyntcomptfOneUnrealM}{431}
\newcommand{\SemmlASemmlSyntcomptfOneUnrealK}{8}
\newcommand{\SemmlASemmlSyntcomptfOneUnrealL}{7}
\newcommand{\SemmlASemmlSyntcomptfOneUnrealScore}{\SemmlASemmlSyntcomptfOneUnrealT[\SemmlASemmlSyntcomptfOneUnrealM+\SemmlASemmlSyntcomptfOneUnrealK/\SemmlASemmlSyntcomptfOneUnrealL]}
\newcommand{\StrixRealSyntcompTwo}{152}
\newcommand{\StrixUnrealSyntcompTwo}{129}
\newcommand{\SemmlARealSyntcompTwo}{162}
\newcommand{\SemmlAUnrealSyntcompTwo}{140}
\newcommand{\SemmlRealSyntcompTwo}{164}
\newcommand{\SemmlUnrealSyntcompTwo}{139}
\newcommand{\trivialSyntcompTwo}{662}
\newcommand{\nontrivialSyntcompTwo}{394}
\newcommand{\trivialStrixSemmlASyntcompTwo}{730}
\newcommand{\unknownStrixSemmlASyntcompTwo}{59}
\newcommand{\StrixSemmlASyntcompTwoAllT}{1.12}
\newcommand{\StrixSemmlASyntcompTwoAllM}{180}
\newcommand{\StrixSemmlASyntcompTwoAllK}{33}
\newcommand{\StrixSemmlASyntcompTwoAllL}{54}
\newcommand{\StrixSemmlASyntcompTwoAllScore}{\StrixSemmlASyntcompTwoAllT[\StrixSemmlASyntcompTwoAllM+\StrixSemmlASyntcompTwoAllK/\StrixSemmlASyntcompTwoAllL]}
\newcommand{\StrixSemmlASyntcompTwoRealT}{1.25}
\newcommand{\StrixSemmlASyntcompTwoRealM}{107}
\newcommand{\StrixSemmlASyntcompTwoRealK}{14}
\newcommand{\StrixSemmlASyntcompTwoRealL}{24}
\newcommand{\StrixSemmlASyntcompTwoRealScore}{\StrixSemmlASyntcompTwoRealT[\StrixSemmlASyntcompTwoRealM+\StrixSemmlASyntcompTwoRealK/\StrixSemmlASyntcompTwoRealL]}
\newcommand{\StrixSemmlASyntcompTwoUnrealT}{0.96}
\newcommand{\StrixSemmlASyntcompTwoUnrealM}{73}
\newcommand{\StrixSemmlASyntcompTwoUnrealK}{19}
\newcommand{\StrixSemmlASyntcompTwoUnrealL}{30}
\newcommand{\StrixSemmlASyntcompTwoUnrealScore}{\StrixSemmlASyntcompTwoUnrealT[\StrixSemmlASyntcompTwoUnrealM+\StrixSemmlASyntcompTwoUnrealK/\StrixSemmlASyntcompTwoUnrealL]}
\newcommand{\trivialStrixSemmlSyntcompTwo}{663}
\newcommand{\unknownStrixSemmlSyntcompTwo}{64}
\newcommand{\StrixSemmlSyntcompTwoAllT}{0.66}
\newcommand{\StrixSemmlSyntcompTwoAllM}{253}
\newcommand{\StrixSemmlSyntcompTwoAllK}{27}
\newcommand{\StrixSemmlSyntcompTwoAllL}{49}
\newcommand{\StrixSemmlSyntcompTwoAllScore}{\StrixSemmlSyntcompTwoAllT[\StrixSemmlSyntcompTwoAllM+\StrixSemmlSyntcompTwoAllK/\StrixSemmlSyntcompTwoAllL]}
\newcommand{\StrixSemmlSyntcompTwoRealT}{0.85}
\newcommand{\StrixSemmlSyntcompTwoRealM}{140}
\newcommand{\StrixSemmlSyntcompTwoRealK}{12}
\newcommand{\StrixSemmlSyntcompTwoRealL}{24}
\newcommand{\StrixSemmlSyntcompTwoRealScore}{\StrixSemmlSyntcompTwoRealT[\StrixSemmlSyntcompTwoRealM+\StrixSemmlSyntcompTwoRealK/\StrixSemmlSyntcompTwoRealL]}
\newcommand{\StrixSemmlSyntcompTwoUnrealT}{0.48}
\newcommand{\StrixSemmlSyntcompTwoUnrealM}{113}
\newcommand{\StrixSemmlSyntcompTwoUnrealK}{15}
\newcommand{\StrixSemmlSyntcompTwoUnrealL}{25}
\newcommand{\StrixSemmlSyntcompTwoUnrealScore}{\StrixSemmlSyntcompTwoUnrealT[\StrixSemmlSyntcompTwoUnrealM+\StrixSemmlSyntcompTwoUnrealK/\StrixSemmlSyntcompTwoUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcompTwo}{663}
\newcommand{\unknownSemmlASemmlSyntcompTwo}{82}
\newcommand{\SemmlASemmlSyntcompTwoAllT}{0.81}
\newcommand{\SemmlASemmlSyntcompTwoAllM}{292}
\newcommand{\SemmlASemmlSyntcompTwoAllK}{9}
\newcommand{\SemmlASemmlSyntcompTwoAllL}{10}
\newcommand{\SemmlASemmlSyntcompTwoAllScore}{\SemmlASemmlSyntcompTwoAllT[\SemmlASemmlSyntcompTwoAllM+\SemmlASemmlSyntcompTwoAllK/\SemmlASemmlSyntcompTwoAllL]}
\newcommand{\SemmlASemmlSyntcompTwoRealT}{0.9}
\newcommand{\SemmlASemmlSyntcompTwoRealM}{160}
\newcommand{\SemmlASemmlSyntcompTwoRealK}{1}
\newcommand{\SemmlASemmlSyntcompTwoRealL}{3}
\newcommand{\SemmlASemmlSyntcompTwoRealScore}{\SemmlASemmlSyntcompTwoRealT[\SemmlASemmlSyntcompTwoRealM+\SemmlASemmlSyntcompTwoRealK/\SemmlASemmlSyntcompTwoRealL]}
\newcommand{\SemmlASemmlSyntcompTwoUnrealT}{0.7}
\newcommand{\SemmlASemmlSyntcompTwoUnrealM}{132}
\newcommand{\SemmlASemmlSyntcompTwoUnrealK}{8}
\newcommand{\SemmlASemmlSyntcompTwoUnrealL}{7}
\newcommand{\SemmlASemmlSyntcompTwoUnrealScore}{\SemmlASemmlSyntcompTwoUnrealT[\SemmlASemmlSyntcompTwoUnrealM+\SemmlASemmlSyntcompTwoUnrealK/\SemmlASemmlSyntcompTwoUnrealL]}
\newcommand{\StrixRealSyntheticTwo}{8}
\newcommand{\StrixUnrealSyntheticTwo}{22}
\newcommand{\SemmlARealSyntheticTwo}{27}
\newcommand{\SemmlAUnrealSyntheticTwo}{40}
\newcommand{\SemmlRealSyntheticTwo}{35}
\newcommand{\SemmlUnrealSyntheticTwo}{48}
\newcommand{\trivialSyntheticTwo}{0}
\newcommand{\nontrivialSyntheticTwo}{200}
\newcommand{\trivialStrixSemmlASyntheticTwo}{0}
\newcommand{\unknownStrixSemmlASyntheticTwo}{133}
\newcommand{\StrixSemmlASyntheticTwoAllT}{9.1}
\newcommand{\StrixSemmlASyntheticTwoAllM}{30}
\newcommand{\StrixSemmlASyntheticTwoAllK}{0}
\newcommand{\StrixSemmlASyntheticTwoAllL}{37}
\newcommand{\StrixSemmlASyntheticTwoAllScore}{\StrixSemmlASyntheticTwoAllT[\StrixSemmlASyntheticTwoAllM+\StrixSemmlASyntheticTwoAllK/\StrixSemmlASyntheticTwoAllL]}
\newcommand{\StrixSemmlASyntheticTwoRealT}{10.44}
\newcommand{\StrixSemmlASyntheticTwoRealM}{8}
\newcommand{\StrixSemmlASyntheticTwoRealK}{0}
\newcommand{\StrixSemmlASyntheticTwoRealL}{19}
\newcommand{\StrixSemmlASyntheticTwoRealScore}{\StrixSemmlASyntheticTwoRealT[\StrixSemmlASyntheticTwoRealM+\StrixSemmlASyntheticTwoRealK/\StrixSemmlASyntheticTwoRealL]}
\newcommand{\StrixSemmlASyntheticTwoUnrealT}{8.66}
\newcommand{\StrixSemmlASyntheticTwoUnrealM}{22}
\newcommand{\StrixSemmlASyntheticTwoUnrealK}{0}
\newcommand{\StrixSemmlASyntheticTwoUnrealL}{18}
\newcommand{\StrixSemmlASyntheticTwoUnrealScore}{\StrixSemmlASyntheticTwoUnrealT[\StrixSemmlASyntheticTwoUnrealM+\StrixSemmlASyntheticTwoUnrealK/\StrixSemmlASyntheticTwoUnrealL]}
\newcommand{\trivialStrixSemmlSyntheticTwo}{0}
\newcommand{\unknownStrixSemmlSyntheticTwo}{117}
\newcommand{\StrixSemmlSyntheticTwoAllT}{8.56}
\newcommand{\StrixSemmlSyntheticTwoAllM}{30}
\newcommand{\StrixSemmlSyntheticTwoAllK}{0}
\newcommand{\StrixSemmlSyntheticTwoAllL}{53}
\newcommand{\StrixSemmlSyntheticTwoAllScore}{\StrixSemmlSyntheticTwoAllT[\StrixSemmlSyntheticTwoAllM+\StrixSemmlSyntheticTwoAllK/\StrixSemmlSyntheticTwoAllL]}
\newcommand{\StrixSemmlSyntheticTwoRealT}{13.07}
\newcommand{\StrixSemmlSyntheticTwoRealM}{8}
\newcommand{\StrixSemmlSyntheticTwoRealK}{0}
\newcommand{\StrixSemmlSyntheticTwoRealL}{27}
\newcommand{\StrixSemmlSyntheticTwoRealScore}{\StrixSemmlSyntheticTwoRealT[\StrixSemmlSyntheticTwoRealM+\StrixSemmlSyntheticTwoRealK/\StrixSemmlSyntheticTwoRealL]}
\newcommand{\StrixSemmlSyntheticTwoUnrealT}{7.33}
\newcommand{\StrixSemmlSyntheticTwoUnrealM}{22}
\newcommand{\StrixSemmlSyntheticTwoUnrealK}{0}
\newcommand{\StrixSemmlSyntheticTwoUnrealL}{26}
\newcommand{\StrixSemmlSyntheticTwoUnrealScore}{\StrixSemmlSyntheticTwoUnrealT[\StrixSemmlSyntheticTwoUnrealM+\StrixSemmlSyntheticTwoUnrealK/\StrixSemmlSyntheticTwoUnrealL]}
\newcommand{\trivialSemmlASemmlSyntheticTwo}{0}
\newcommand{\unknownSemmlASemmlSyntheticTwo}{113}
\newcommand{\SemmlASemmlSyntheticTwoAllT}{1.36}
\newcommand{\SemmlASemmlSyntheticTwoAllM}{63}
\newcommand{\SemmlASemmlSyntheticTwoAllK}{4}
\newcommand{\SemmlASemmlSyntheticTwoAllL}{20}
\newcommand{\SemmlASemmlSyntheticTwoAllScore}{\SemmlASemmlSyntheticTwoAllT[\SemmlASemmlSyntheticTwoAllM+\SemmlASemmlSyntheticTwoAllK/\SemmlASemmlSyntheticTwoAllL]}
\newcommand{\SemmlASemmlSyntheticTwoRealT}{1.67}
\newcommand{\SemmlASemmlSyntheticTwoRealM}{25}
\newcommand{\SemmlASemmlSyntheticTwoRealK}{2}
\newcommand{\SemmlASemmlSyntheticTwoRealL}{10}
\newcommand{\SemmlASemmlSyntheticTwoRealScore}{\SemmlASemmlSyntheticTwoRealT[\SemmlASemmlSyntheticTwoRealM+\SemmlASemmlSyntheticTwoRealK/\SemmlASemmlSyntheticTwoRealL]}
\newcommand{\SemmlASemmlSyntheticTwoUnrealT}{1.19}
\newcommand{\SemmlASemmlSyntheticTwoUnrealM}{38}
\newcommand{\SemmlASemmlSyntheticTwoUnrealK}{2}
\newcommand{\SemmlASemmlSyntheticTwoUnrealL}{10}
\newcommand{\SemmlASemmlSyntheticTwoUnrealScore}{\SemmlASemmlSyntheticTwoUnrealT[\SemmlASemmlSyntheticTwoUnrealM+\SemmlASemmlSyntheticTwoUnrealK/\SemmlASemmlSyntheticTwoUnrealL]}
\newcommand{\StrixRealSyntcomptfTwo}{174}
\newcommand{\StrixUnrealSyntcomptfTwo}{135}
\newcommand{\SemmlARealSyntcomptfTwo}{184}
\newcommand{\SemmlAUnrealSyntcomptfTwo}{146}
\newcommand{\SemmlRealSyntcomptfTwo}{186}
\newcommand{\SemmlUnrealSyntcomptfTwo}{145}
\newcommand{\trivialSyntcomptfTwo}{669}
\newcommand{\nontrivialSyntcomptfTwo}{442}
\newcommand{\trivialStrixSemmlASyntcomptfTwo}{741}
\newcommand{\unknownStrixSemmlASyntcomptfTwo}{79}
\newcommand{\StrixSemmlASyntcomptfTwoAllT}{1.13}
\newcommand{\StrixSemmlASyntcomptfTwoAllM}{204}
\newcommand{\StrixSemmlASyntcomptfTwoAllK}{33}
\newcommand{\StrixSemmlASyntcomptfTwoAllL}{54}
\newcommand{\StrixSemmlASyntcomptfTwoAllScore}{\StrixSemmlASyntcomptfTwoAllT[\StrixSemmlASyntcomptfTwoAllM+\StrixSemmlASyntcomptfTwoAllK/\StrixSemmlASyntcomptfTwoAllL]}
\newcommand{\StrixSemmlASyntcomptfTwoRealT}{1.24}
\newcommand{\StrixSemmlASyntcomptfTwoRealM}{126}
\newcommand{\StrixSemmlASyntcomptfTwoRealK}{14}
\newcommand{\StrixSemmlASyntcomptfTwoRealL}{24}
\newcommand{\StrixSemmlASyntcomptfTwoRealScore}{\StrixSemmlASyntcomptfTwoRealT[\StrixSemmlASyntcomptfTwoRealM+\StrixSemmlASyntcomptfTwoRealK/\StrixSemmlASyntcomptfTwoRealL]}
\newcommand{\StrixSemmlASyntcomptfTwoUnrealT}{0.97}
\newcommand{\StrixSemmlASyntcomptfTwoUnrealM}{78}
\newcommand{\StrixSemmlASyntcomptfTwoUnrealK}{19}
\newcommand{\StrixSemmlASyntcomptfTwoUnrealL}{30}
\newcommand{\StrixSemmlASyntcomptfTwoUnrealScore}{\StrixSemmlASyntcomptfTwoUnrealT[\StrixSemmlASyntcomptfTwoUnrealM+\StrixSemmlASyntcomptfTwoUnrealK/\StrixSemmlASyntcomptfTwoUnrealL]}
\newcommand{\trivialStrixSemmlSyntcomptfTwo}{670}
\newcommand{\unknownStrixSemmlSyntcomptfTwo}{84}
\newcommand{\StrixSemmlSyntcomptfTwoAllT}{0.67}
\newcommand{\StrixSemmlSyntcomptfTwoAllM}{281}
\newcommand{\StrixSemmlSyntcomptfTwoAllK}{27}
\newcommand{\StrixSemmlSyntcomptfTwoAllL}{49}
\newcommand{\StrixSemmlSyntcomptfTwoAllScore}{\StrixSemmlSyntcomptfTwoAllT[\StrixSemmlSyntcomptfTwoAllM+\StrixSemmlSyntcomptfTwoAllK/\StrixSemmlSyntcomptfTwoAllL]}
\newcommand{\StrixSemmlSyntcomptfTwoRealT}{0.85}
\newcommand{\StrixSemmlSyntcomptfTwoRealM}{162}
\newcommand{\StrixSemmlSyntcomptfTwoRealK}{12}
\newcommand{\StrixSemmlSyntcomptfTwoRealL}{24}
\newcommand{\StrixSemmlSyntcomptfTwoRealScore}{\StrixSemmlSyntcomptfTwoRealT[\StrixSemmlSyntcomptfTwoRealM+\StrixSemmlSyntcomptfTwoRealK/\StrixSemmlSyntcomptfTwoRealL]}
\newcommand{\StrixSemmlSyntcomptfTwoUnrealT}{0.49}
\newcommand{\StrixSemmlSyntcomptfTwoUnrealM}{119}
\newcommand{\StrixSemmlSyntcomptfTwoUnrealK}{15}
\newcommand{\StrixSemmlSyntcomptfTwoUnrealL}{25}
\newcommand{\StrixSemmlSyntcomptfTwoUnrealScore}{\StrixSemmlSyntcomptfTwoUnrealT[\StrixSemmlSyntcomptfTwoUnrealM+\StrixSemmlSyntcomptfTwoUnrealK/\StrixSemmlSyntcomptfTwoUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcomptfTwo}{670}
\newcommand{\unknownSemmlASemmlSyntcomptfTwo}{102}
\newcommand{\SemmlASemmlSyntcomptfTwoAllT}{0.8}
\newcommand{\SemmlASemmlSyntcomptfTwoAllM}{320}
\newcommand{\SemmlASemmlSyntcomptfTwoAllK}{9}
\newcommand{\SemmlASemmlSyntcomptfTwoAllL}{10}
\newcommand{\SemmlASemmlSyntcomptfTwoAllScore}{\SemmlASemmlSyntcomptfTwoAllT[\SemmlASemmlSyntcomptfTwoAllM+\SemmlASemmlSyntcomptfTwoAllK/\SemmlASemmlSyntcomptfTwoAllL]}
\newcommand{\SemmlASemmlSyntcomptfTwoRealT}{0.89}
\newcommand{\SemmlASemmlSyntcomptfTwoRealM}{182}
\newcommand{\SemmlASemmlSyntcomptfTwoRealK}{1}
\newcommand{\SemmlASemmlSyntcomptfTwoRealL}{3}
\newcommand{\SemmlASemmlSyntcomptfTwoRealScore}{\SemmlASemmlSyntcomptfTwoRealT[\SemmlASemmlSyntcomptfTwoRealM+\SemmlASemmlSyntcomptfTwoRealK/\SemmlASemmlSyntcomptfTwoRealL]}
\newcommand{\SemmlASemmlSyntcomptfTwoUnrealT}{0.7}
\newcommand{\SemmlASemmlSyntcomptfTwoUnrealM}{138}
\newcommand{\SemmlASemmlSyntcomptfTwoUnrealK}{8}
\newcommand{\SemmlASemmlSyntcomptfTwoUnrealL}{7}
\newcommand{\SemmlASemmlSyntcomptfTwoUnrealScore}{\SemmlASemmlSyntcomptfTwoUnrealT[\SemmlASemmlSyntcomptfTwoUnrealM+\SemmlASemmlSyntcomptfTwoUnrealK/\SemmlASemmlSyntcomptfTwoUnrealL]}
\newcommand{\StrixRealSyntcompFive}{99}
\newcommand{\StrixUnrealSyntcompFive}{70}
\newcommand{\SemmlARealSyntcompFive}{109}
\newcommand{\SemmlAUnrealSyntcompFive}{81}
\newcommand{\SemmlRealSyntcompFive}{111}
\newcommand{\SemmlUnrealSyntcompFive}{80}
\newcommand{\trivialSyntcompFive}{774}
\newcommand{\nontrivialSyntcompFive}{282}
\newcommand{\trivialStrixSemmlASyntcompFive}{783}
\newcommand{\unknownStrixSemmlASyntcompFive}{59}
\newcommand{\StrixSemmlASyntcompFiveAllT}{1.47}
\newcommand{\StrixSemmlASyntcompFiveAllM}{127}
\newcommand{\StrixSemmlASyntcompFiveAllK}{33}
\newcommand{\StrixSemmlASyntcompFiveAllL}{54}
\newcommand{\StrixSemmlASyntcompFiveAllScore}{\StrixSemmlASyntcompFiveAllT[\StrixSemmlASyntcompFiveAllM+\StrixSemmlASyntcompFiveAllK/\StrixSemmlASyntcompFiveAllL]}
\newcommand{\StrixSemmlASyntcompFiveRealT}{1.52}
\newcommand{\StrixSemmlASyntcompFiveRealM}{82}
\newcommand{\StrixSemmlASyntcompFiveRealK}{14}
\newcommand{\StrixSemmlASyntcompFiveRealL}{24}
\newcommand{\StrixSemmlASyntcompFiveRealScore}{\StrixSemmlASyntcompFiveRealT[\StrixSemmlASyntcompFiveRealM+\StrixSemmlASyntcompFiveRealK/\StrixSemmlASyntcompFiveRealL]}
\newcommand{\StrixSemmlASyntcompFiveUnrealT}{1.38}
\newcommand{\StrixSemmlASyntcompFiveUnrealM}{45}
\newcommand{\StrixSemmlASyntcompFiveUnrealK}{19}
\newcommand{\StrixSemmlASyntcompFiveUnrealL}{30}
\newcommand{\StrixSemmlASyntcompFiveUnrealScore}{\StrixSemmlASyntcompFiveUnrealT[\StrixSemmlASyntcompFiveUnrealM+\StrixSemmlASyntcompFiveUnrealK/\StrixSemmlASyntcompFiveUnrealL]}
\newcommand{\trivialStrixSemmlSyntcompFive}{787}
\newcommand{\unknownStrixSemmlSyntcompFive}{64}
\newcommand{\StrixSemmlSyntcompFiveAllT}{1.4}
\newcommand{\StrixSemmlSyntcompFiveAllM}{129}
\newcommand{\StrixSemmlSyntcompFiveAllK}{27}
\newcommand{\StrixSemmlSyntcompFiveAllL}{49}
\newcommand{\StrixSemmlSyntcompFiveAllScore}{\StrixSemmlSyntcompFiveAllT[\StrixSemmlSyntcompFiveAllM+\StrixSemmlSyntcompFiveAllK/\StrixSemmlSyntcompFiveAllL]}
\newcommand{\StrixSemmlSyntcompFiveRealT}{1.88}
\newcommand{\StrixSemmlSyntcompFiveRealM}{75}
\newcommand{\StrixSemmlSyntcompFiveRealK}{12}
\newcommand{\StrixSemmlSyntcompFiveRealL}{24}
\newcommand{\StrixSemmlSyntcompFiveRealScore}{\StrixSemmlSyntcompFiveRealT[\StrixSemmlSyntcompFiveRealM+\StrixSemmlSyntcompFiveRealK/\StrixSemmlSyntcompFiveRealL]}
\newcommand{\StrixSemmlSyntcompFiveUnrealT}{0.92}
\newcommand{\StrixSemmlSyntcompFiveUnrealM}{54}
\newcommand{\StrixSemmlSyntcompFiveUnrealK}{15}
\newcommand{\StrixSemmlSyntcompFiveUnrealL}{25}
\newcommand{\StrixSemmlSyntcompFiveUnrealScore}{\StrixSemmlSyntcompFiveUnrealT[\StrixSemmlSyntcompFiveUnrealM+\StrixSemmlSyntcompFiveUnrealK/\StrixSemmlSyntcompFiveUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcompFive}{780}
\newcommand{\unknownSemmlASemmlSyntcompFive}{82}
\newcommand{\SemmlASemmlSyntcompFiveAllT}{0.91}
\newcommand{\SemmlASemmlSyntcompFiveAllM}{175}
\newcommand{\SemmlASemmlSyntcompFiveAllK}{9}
\newcommand{\SemmlASemmlSyntcompFiveAllL}{10}
\newcommand{\SemmlASemmlSyntcompFiveAllScore}{\SemmlASemmlSyntcompFiveAllT[\SemmlASemmlSyntcompFiveAllM+\SemmlASemmlSyntcompFiveAllK/\SemmlASemmlSyntcompFiveAllL]}
\newcommand{\SemmlASemmlSyntcompFiveRealT}{1.04}
\newcommand{\SemmlASemmlSyntcompFiveRealM}{104}
\newcommand{\SemmlASemmlSyntcompFiveRealK}{1}
\newcommand{\SemmlASemmlSyntcompFiveRealL}{3}
\newcommand{\SemmlASemmlSyntcompFiveRealScore}{\SemmlASemmlSyntcompFiveRealT[\SemmlASemmlSyntcompFiveRealM+\SemmlASemmlSyntcompFiveRealK/\SemmlASemmlSyntcompFiveRealL]}
\newcommand{\SemmlASemmlSyntcompFiveUnrealT}{0.75}
\newcommand{\SemmlASemmlSyntcompFiveUnrealM}{71}
\newcommand{\SemmlASemmlSyntcompFiveUnrealK}{8}
\newcommand{\SemmlASemmlSyntcompFiveUnrealL}{7}
\newcommand{\SemmlASemmlSyntcompFiveUnrealScore}{\SemmlASemmlSyntcompFiveUnrealT[\SemmlASemmlSyntcompFiveUnrealM+\SemmlASemmlSyntcompFiveUnrealK/\SemmlASemmlSyntcompFiveUnrealL]}
\newcommand{\StrixRealSyntheticFive}{8}
\newcommand{\StrixUnrealSyntheticFive}{22}
\newcommand{\SemmlARealSyntheticFive}{27}
\newcommand{\SemmlAUnrealSyntheticFive}{40}
\newcommand{\SemmlRealSyntheticFive}{35}
\newcommand{\SemmlUnrealSyntheticFive}{48}
\newcommand{\trivialSyntheticFive}{0}
\newcommand{\nontrivialSyntheticFive}{200}
\newcommand{\trivialStrixSemmlASyntheticFive}{0}
\newcommand{\unknownStrixSemmlASyntheticFive}{133}
\newcommand{\StrixSemmlASyntheticFiveAllT}{9.1}
\newcommand{\StrixSemmlASyntheticFiveAllM}{30}
\newcommand{\StrixSemmlASyntheticFiveAllK}{0}
\newcommand{\StrixSemmlASyntheticFiveAllL}{37}
\newcommand{\StrixSemmlASyntheticFiveAllScore}{\StrixSemmlASyntheticFiveAllT[\StrixSemmlASyntheticFiveAllM+\StrixSemmlASyntheticFiveAllK/\StrixSemmlASyntheticFiveAllL]}
\newcommand{\StrixSemmlASyntheticFiveRealT}{10.44}
\newcommand{\StrixSemmlASyntheticFiveRealM}{8}
\newcommand{\StrixSemmlASyntheticFiveRealK}{0}
\newcommand{\StrixSemmlASyntheticFiveRealL}{19}
\newcommand{\StrixSemmlASyntheticFiveRealScore}{\StrixSemmlASyntheticFiveRealT[\StrixSemmlASyntheticFiveRealM+\StrixSemmlASyntheticFiveRealK/\StrixSemmlASyntheticFiveRealL]}
\newcommand{\StrixSemmlASyntheticFiveUnrealT}{8.66}
\newcommand{\StrixSemmlASyntheticFiveUnrealM}{22}
\newcommand{\StrixSemmlASyntheticFiveUnrealK}{0}
\newcommand{\StrixSemmlASyntheticFiveUnrealL}{18}
\newcommand{\StrixSemmlASyntheticFiveUnrealScore}{\StrixSemmlASyntheticFiveUnrealT[\StrixSemmlASyntheticFiveUnrealM+\StrixSemmlASyntheticFiveUnrealK/\StrixSemmlASyntheticFiveUnrealL]}
\newcommand{\trivialStrixSemmlSyntheticFive}{0}
\newcommand{\unknownStrixSemmlSyntheticFive}{117}
\newcommand{\StrixSemmlSyntheticFiveAllT}{8.56}
\newcommand{\StrixSemmlSyntheticFiveAllM}{30}
\newcommand{\StrixSemmlSyntheticFiveAllK}{0}
\newcommand{\StrixSemmlSyntheticFiveAllL}{53}
\newcommand{\StrixSemmlSyntheticFiveAllScore}{\StrixSemmlSyntheticFiveAllT[\StrixSemmlSyntheticFiveAllM+\StrixSemmlSyntheticFiveAllK/\StrixSemmlSyntheticFiveAllL]}
\newcommand{\StrixSemmlSyntheticFiveRealT}{13.07}
\newcommand{\StrixSemmlSyntheticFiveRealM}{8}
\newcommand{\StrixSemmlSyntheticFiveRealK}{0}
\newcommand{\StrixSemmlSyntheticFiveRealL}{27}
\newcommand{\StrixSemmlSyntheticFiveRealScore}{\StrixSemmlSyntheticFiveRealT[\StrixSemmlSyntheticFiveRealM+\StrixSemmlSyntheticFiveRealK/\StrixSemmlSyntheticFiveRealL]}
\newcommand{\StrixSemmlSyntheticFiveUnrealT}{7.33}
\newcommand{\StrixSemmlSyntheticFiveUnrealM}{22}
\newcommand{\StrixSemmlSyntheticFiveUnrealK}{0}
\newcommand{\StrixSemmlSyntheticFiveUnrealL}{26}
\newcommand{\StrixSemmlSyntheticFiveUnrealScore}{\StrixSemmlSyntheticFiveUnrealT[\StrixSemmlSyntheticFiveUnrealM+\StrixSemmlSyntheticFiveUnrealK/\StrixSemmlSyntheticFiveUnrealL]}
\newcommand{\trivialSemmlASemmlSyntheticFive}{1}
\newcommand{\unknownSemmlASemmlSyntheticFive}{113}
\newcommand{\SemmlASemmlSyntheticFiveAllT}{1.38}
\newcommand{\SemmlASemmlSyntheticFiveAllM}{62}
\newcommand{\SemmlASemmlSyntheticFiveAllK}{4}
\newcommand{\SemmlASemmlSyntheticFiveAllL}{20}
\newcommand{\SemmlASemmlSyntheticFiveAllScore}{\SemmlASemmlSyntheticFiveAllT[\SemmlASemmlSyntheticFiveAllM+\SemmlASemmlSyntheticFiveAllK/\SemmlASemmlSyntheticFiveAllL]}
\newcommand{\SemmlASemmlSyntheticFiveRealT}{1.67}
\newcommand{\SemmlASemmlSyntheticFiveRealM}{25}
\newcommand{\SemmlASemmlSyntheticFiveRealK}{2}
\newcommand{\SemmlASemmlSyntheticFiveRealL}{10}
\newcommand{\SemmlASemmlSyntheticFiveRealScore}{\SemmlASemmlSyntheticFiveRealT[\SemmlASemmlSyntheticFiveRealM+\SemmlASemmlSyntheticFiveRealK/\SemmlASemmlSyntheticFiveRealL]}
\newcommand{\SemmlASemmlSyntheticFiveUnrealT}{1.21}
\newcommand{\SemmlASemmlSyntheticFiveUnrealM}{37}
\newcommand{\SemmlASemmlSyntheticFiveUnrealK}{2}
\newcommand{\SemmlASemmlSyntheticFiveUnrealL}{10}
\newcommand{\SemmlASemmlSyntheticFiveUnrealScore}{\SemmlASemmlSyntheticFiveUnrealT[\SemmlASemmlSyntheticFiveUnrealM+\SemmlASemmlSyntheticFiveUnrealK/\SemmlASemmlSyntheticFiveUnrealL]}
\newcommand{\StrixRealSyntcomptfFive}{115}
\newcommand{\StrixUnrealSyntcomptfFive}{73}
\newcommand{\SemmlARealSyntcomptfFive}{125}
\newcommand{\SemmlAUnrealSyntcomptfFive}{84}
\newcommand{\SemmlRealSyntcomptfFive}{127}
\newcommand{\SemmlUnrealSyntcomptfFive}{83}
\newcommand{\trivialSyntcomptfFive}{790}
\newcommand{\nontrivialSyntcomptfFive}{321}
\newcommand{\trivialStrixSemmlASyntcomptfFive}{799}
\newcommand{\unknownStrixSemmlASyntcomptfFive}{79}
\newcommand{\StrixSemmlASyntcomptfFiveAllT}{1.47}
\newcommand{\StrixSemmlASyntcomptfFiveAllM}{146}
\newcommand{\StrixSemmlASyntcomptfFiveAllK}{33}
\newcommand{\StrixSemmlASyntcomptfFiveAllL}{54}
\newcommand{\StrixSemmlASyntcomptfFiveAllScore}{\StrixSemmlASyntcomptfFiveAllT[\StrixSemmlASyntcomptfFiveAllM+\StrixSemmlASyntcomptfFiveAllK/\StrixSemmlASyntcomptfFiveAllL]}
\newcommand{\StrixSemmlASyntcomptfFiveRealT}{1.5}
\newcommand{\StrixSemmlASyntcomptfFiveRealM}{98}
\newcommand{\StrixSemmlASyntcomptfFiveRealK}{14}
\newcommand{\StrixSemmlASyntcomptfFiveRealL}{24}
\newcommand{\StrixSemmlASyntcomptfFiveRealScore}{\StrixSemmlASyntcomptfFiveRealT[\StrixSemmlASyntcomptfFiveRealM+\StrixSemmlASyntcomptfFiveRealK/\StrixSemmlASyntcomptfFiveRealL]}
\newcommand{\StrixSemmlASyntcomptfFiveUnrealT}{1.42}
\newcommand{\StrixSemmlASyntcomptfFiveUnrealM}{48}
\newcommand{\StrixSemmlASyntcomptfFiveUnrealK}{19}
\newcommand{\StrixSemmlASyntcomptfFiveUnrealL}{30}
\newcommand{\StrixSemmlASyntcomptfFiveUnrealScore}{\StrixSemmlASyntcomptfFiveUnrealT[\StrixSemmlASyntcomptfFiveUnrealM+\StrixSemmlASyntcomptfFiveUnrealK/\StrixSemmlASyntcomptfFiveUnrealL]}
\newcommand{\trivialStrixSemmlSyntcomptfFive}{803}
\newcommand{\unknownStrixSemmlSyntcomptfFive}{84}
\newcommand{\StrixSemmlSyntcomptfFiveAllT}{1.37}
\newcommand{\StrixSemmlSyntcomptfFiveAllM}{148}
\newcommand{\StrixSemmlSyntcomptfFiveAllK}{27}
\newcommand{\StrixSemmlSyntcomptfFiveAllL}{49}
\newcommand{\StrixSemmlSyntcomptfFiveAllScore}{\StrixSemmlSyntcomptfFiveAllT[\StrixSemmlSyntcomptfFiveAllM+\StrixSemmlSyntcomptfFiveAllK/\StrixSemmlSyntcomptfFiveAllL]}
\newcommand{\StrixSemmlSyntcomptfFiveRealT}{1.73}
\newcommand{\StrixSemmlSyntcomptfFiveRealM}{91}
\newcommand{\StrixSemmlSyntcomptfFiveRealK}{12}
\newcommand{\StrixSemmlSyntcomptfFiveRealL}{24}
\newcommand{\StrixSemmlSyntcomptfFiveRealScore}{\StrixSemmlSyntcomptfFiveRealT[\StrixSemmlSyntcomptfFiveRealM+\StrixSemmlSyntcomptfFiveRealK/\StrixSemmlSyntcomptfFiveRealL]}
\newcommand{\StrixSemmlSyntcomptfFiveUnrealT}{0.95}
\newcommand{\StrixSemmlSyntcomptfFiveUnrealM}{57}
\newcommand{\StrixSemmlSyntcomptfFiveUnrealK}{15}
\newcommand{\StrixSemmlSyntcomptfFiveUnrealL}{25}
\newcommand{\StrixSemmlSyntcomptfFiveUnrealScore}{\StrixSemmlSyntcomptfFiveUnrealT[\StrixSemmlSyntcomptfFiveUnrealM+\StrixSemmlSyntcomptfFiveUnrealK/\StrixSemmlSyntcomptfFiveUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcomptfFive}{796}
\newcommand{\unknownSemmlASemmlSyntcomptfFive}{102}
\newcommand{\SemmlASemmlSyntcomptfFiveAllT}{0.9}
\newcommand{\SemmlASemmlSyntcomptfFiveAllM}{194}
\newcommand{\SemmlASemmlSyntcomptfFiveAllK}{9}
\newcommand{\SemmlASemmlSyntcomptfFiveAllL}{10}
\newcommand{\SemmlASemmlSyntcomptfFiveAllScore}{\SemmlASemmlSyntcomptfFiveAllT[\SemmlASemmlSyntcomptfFiveAllM+\SemmlASemmlSyntcomptfFiveAllK/\SemmlASemmlSyntcomptfFiveAllL]}
\newcommand{\SemmlASemmlSyntcomptfFiveRealT}{1.01}
\newcommand{\SemmlASemmlSyntcomptfFiveRealM}{120}
\newcommand{\SemmlASemmlSyntcomptfFiveRealK}{1}
\newcommand{\SemmlASemmlSyntcomptfFiveRealL}{3}
\newcommand{\SemmlASemmlSyntcomptfFiveRealScore}{\SemmlASemmlSyntcomptfFiveRealT[\SemmlASemmlSyntcomptfFiveRealM+\SemmlASemmlSyntcomptfFiveRealK/\SemmlASemmlSyntcomptfFiveRealL]}
\newcommand{\SemmlASemmlSyntcomptfFiveUnrealT}{0.75}
\newcommand{\SemmlASemmlSyntcomptfFiveUnrealM}{74}
\newcommand{\SemmlASemmlSyntcomptfFiveUnrealK}{8}
\newcommand{\SemmlASemmlSyntcomptfFiveUnrealL}{7}
\newcommand{\SemmlASemmlSyntcomptfFiveUnrealScore}{\SemmlASemmlSyntcomptfFiveUnrealT[\SemmlASemmlSyntcomptfFiveUnrealM+\SemmlASemmlSyntcomptfFiveUnrealK/\SemmlASemmlSyntcomptfFiveUnrealL]}
\newcommand{\StrixRealSyntcompTen}{84}
\newcommand{\StrixUnrealSyntcompTen}{60}
\newcommand{\SemmlARealSyntcompTen}{94}
\newcommand{\SemmlAUnrealSyntcompTen}{71}
\newcommand{\SemmlRealSyntcompTen}{96}
\newcommand{\SemmlUnrealSyntcompTen}{70}
\newcommand{\trivialSyntcompTen}{799}
\newcommand{\nontrivialSyntcompTen}{257}
\newcommand{\trivialStrixSemmlASyntcompTen}{806}
\newcommand{\unknownStrixSemmlASyntcompTen}{59}
\newcommand{\StrixSemmlASyntcompTenAllT}{1.72}
\newcommand{\StrixSemmlASyntcompTenAllM}{104}
\newcommand{\StrixSemmlASyntcompTenAllK}{33}
\newcommand{\StrixSemmlASyntcompTenAllL}{54}
\newcommand{\StrixSemmlASyntcompTenAllScore}{\StrixSemmlASyntcompTenAllT[\StrixSemmlASyntcompTenAllM+\StrixSemmlASyntcompTenAllK/\StrixSemmlASyntcompTenAllL]}
\newcommand{\StrixSemmlASyntcompTenRealT}{1.68}
\newcommand{\StrixSemmlASyntcompTenRealM}{69}
\newcommand{\StrixSemmlASyntcompTenRealK}{14}
\newcommand{\StrixSemmlASyntcompTenRealL}{24}
\newcommand{\StrixSemmlASyntcompTenRealScore}{\StrixSemmlASyntcompTenRealT[\StrixSemmlASyntcompTenRealM+\StrixSemmlASyntcompTenRealK/\StrixSemmlASyntcompTenRealL]}
\newcommand{\StrixSemmlASyntcompTenUnrealT}{1.81}
\newcommand{\StrixSemmlASyntcompTenUnrealM}{35}
\newcommand{\StrixSemmlASyntcompTenUnrealK}{19}
\newcommand{\StrixSemmlASyntcompTenUnrealL}{30}
\newcommand{\StrixSemmlASyntcompTenUnrealScore}{\StrixSemmlASyntcompTenUnrealT[\StrixSemmlASyntcompTenUnrealM+\StrixSemmlASyntcompTenUnrealK/\StrixSemmlASyntcompTenUnrealL]}
\newcommand{\trivialStrixSemmlSyntcompTen}{815}
\newcommand{\unknownStrixSemmlSyntcompTen}{64}
\newcommand{\StrixSemmlSyntcompTenAllT}{1.9}
\newcommand{\StrixSemmlSyntcompTenAllM}{101}
\newcommand{\StrixSemmlSyntcompTenAllK}{27}
\newcommand{\StrixSemmlSyntcompTenAllL}{49}
\newcommand{\StrixSemmlSyntcompTenAllScore}{\StrixSemmlSyntcompTenAllT[\StrixSemmlSyntcompTenAllM+\StrixSemmlSyntcompTenAllK/\StrixSemmlSyntcompTenAllL]}
\newcommand{\StrixSemmlSyntcompTenRealT}{2.35}
\newcommand{\StrixSemmlSyntcompTenRealM}{61}
\newcommand{\StrixSemmlSyntcompTenRealK}{12}
\newcommand{\StrixSemmlSyntcompTenRealL}{24}
\newcommand{\StrixSemmlSyntcompTenRealScore}{\StrixSemmlSyntcompTenRealT[\StrixSemmlSyntcompTenRealM+\StrixSemmlSyntcompTenRealK/\StrixSemmlSyntcompTenRealL]}
\newcommand{\StrixSemmlSyntcompTenUnrealT}{1.37}
\newcommand{\StrixSemmlSyntcompTenUnrealM}{40}
\newcommand{\StrixSemmlSyntcompTenUnrealK}{15}
\newcommand{\StrixSemmlSyntcompTenUnrealL}{25}
\newcommand{\StrixSemmlSyntcompTenUnrealScore}{\StrixSemmlSyntcompTenUnrealT[\StrixSemmlSyntcompTenUnrealM+\StrixSemmlSyntcompTenUnrealK/\StrixSemmlSyntcompTenUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcompTen}{815}
\newcommand{\unknownSemmlASemmlSyntcompTen}{82}
\newcommand{\SemmlASemmlSyntcompTenAllT}{0.94}
\newcommand{\SemmlASemmlSyntcompTenAllM}{140}
\newcommand{\SemmlASemmlSyntcompTenAllK}{9}
\newcommand{\SemmlASemmlSyntcompTenAllL}{10}
\newcommand{\SemmlASemmlSyntcompTenAllScore}{\SemmlASemmlSyntcompTenAllT[\SemmlASemmlSyntcompTenAllM+\SemmlASemmlSyntcompTenAllK/\SemmlASemmlSyntcompTenAllL]}
\newcommand{\SemmlASemmlSyntcompTenRealT}{1.08}
\newcommand{\SemmlASemmlSyntcompTenRealM}{82}
\newcommand{\SemmlASemmlSyntcompTenRealK}{1}
\newcommand{\SemmlASemmlSyntcompTenRealL}{3}
\newcommand{\SemmlASemmlSyntcompTenRealScore}{\SemmlASemmlSyntcompTenRealT[\SemmlASemmlSyntcompTenRealM+\SemmlASemmlSyntcompTenRealK/\SemmlASemmlSyntcompTenRealL]}
\newcommand{\SemmlASemmlSyntcompTenUnrealT}{0.77}
\newcommand{\SemmlASemmlSyntcompTenUnrealM}{58}
\newcommand{\SemmlASemmlSyntcompTenUnrealK}{8}
\newcommand{\SemmlASemmlSyntcompTenUnrealL}{7}
\newcommand{\SemmlASemmlSyntcompTenUnrealScore}{\SemmlASemmlSyntcompTenUnrealT[\SemmlASemmlSyntcompTenUnrealM+\SemmlASemmlSyntcompTenUnrealK/\SemmlASemmlSyntcompTenUnrealL]}
\newcommand{\StrixRealSyntheticTen}{8}
\newcommand{\StrixUnrealSyntheticTen}{22}
\newcommand{\SemmlARealSyntheticTen}{27}
\newcommand{\SemmlAUnrealSyntheticTen}{40}
\newcommand{\SemmlRealSyntheticTen}{35}
\newcommand{\SemmlUnrealSyntheticTen}{48}
\newcommand{\trivialSyntheticTen}{0}
\newcommand{\nontrivialSyntheticTen}{200}
\newcommand{\trivialStrixSemmlASyntheticTen}{1}
\newcommand{\unknownStrixSemmlASyntheticTen}{133}
\newcommand{\StrixSemmlASyntheticTenAllT}{9.53}
\newcommand{\StrixSemmlASyntheticTenAllM}{29}
\newcommand{\StrixSemmlASyntheticTenAllK}{0}
\newcommand{\StrixSemmlASyntheticTenAllL}{37}
\newcommand{\StrixSemmlASyntheticTenAllScore}{\StrixSemmlASyntheticTenAllT[\StrixSemmlASyntheticTenAllM+\StrixSemmlASyntheticTenAllK/\StrixSemmlASyntheticTenAllL]}
\newcommand{\StrixSemmlASyntheticTenRealT}{10.44}
\newcommand{\StrixSemmlASyntheticTenRealM}{8}
\newcommand{\StrixSemmlASyntheticTenRealK}{0}
\newcommand{\StrixSemmlASyntheticTenRealL}{19}
\newcommand{\StrixSemmlASyntheticTenRealScore}{\StrixSemmlASyntheticTenRealT[\StrixSemmlASyntheticTenRealM+\StrixSemmlASyntheticTenRealK/\StrixSemmlASyntheticTenRealL]}
\newcommand{\StrixSemmlASyntheticTenUnrealT}{9.2}
\newcommand{\StrixSemmlASyntheticTenUnrealM}{21}
\newcommand{\StrixSemmlASyntheticTenUnrealK}{0}
\newcommand{\StrixSemmlASyntheticTenUnrealL}{18}
\newcommand{\StrixSemmlASyntheticTenUnrealScore}{\StrixSemmlASyntheticTenUnrealT[\StrixSemmlASyntheticTenUnrealM+\StrixSemmlASyntheticTenUnrealK/\StrixSemmlASyntheticTenUnrealL]}
\newcommand{\trivialStrixSemmlSyntheticTen}{0}
\newcommand{\unknownStrixSemmlSyntheticTen}{117}
\newcommand{\StrixSemmlSyntheticTenAllT}{8.56}
\newcommand{\StrixSemmlSyntheticTenAllM}{30}
\newcommand{\StrixSemmlSyntheticTenAllK}{0}
\newcommand{\StrixSemmlSyntheticTenAllL}{53}
\newcommand{\StrixSemmlSyntheticTenAllScore}{\StrixSemmlSyntheticTenAllT[\StrixSemmlSyntheticTenAllM+\StrixSemmlSyntheticTenAllK/\StrixSemmlSyntheticTenAllL]}
\newcommand{\StrixSemmlSyntheticTenRealT}{13.07}
\newcommand{\StrixSemmlSyntheticTenRealM}{8}
\newcommand{\StrixSemmlSyntheticTenRealK}{0}
\newcommand{\StrixSemmlSyntheticTenRealL}{27}
\newcommand{\StrixSemmlSyntheticTenRealScore}{\StrixSemmlSyntheticTenRealT[\StrixSemmlSyntheticTenRealM+\StrixSemmlSyntheticTenRealK/\StrixSemmlSyntheticTenRealL]}
\newcommand{\StrixSemmlSyntheticTenUnrealT}{7.33}
\newcommand{\StrixSemmlSyntheticTenUnrealM}{22}
\newcommand{\StrixSemmlSyntheticTenUnrealK}{0}
\newcommand{\StrixSemmlSyntheticTenUnrealL}{26}
\newcommand{\StrixSemmlSyntheticTenUnrealScore}{\StrixSemmlSyntheticTenUnrealT[\StrixSemmlSyntheticTenUnrealM+\StrixSemmlSyntheticTenUnrealK/\StrixSemmlSyntheticTenUnrealL]}
\newcommand{\trivialSemmlASemmlSyntheticTen}{7}
\newcommand{\unknownSemmlASemmlSyntheticTen}{113}
\newcommand{\SemmlASemmlSyntheticTenAllT}{1.42}
\newcommand{\SemmlASemmlSyntheticTenAllM}{56}
\newcommand{\SemmlASemmlSyntheticTenAllK}{4}
\newcommand{\SemmlASemmlSyntheticTenAllL}{20}
\newcommand{\SemmlASemmlSyntheticTenAllScore}{\SemmlASemmlSyntheticTenAllT[\SemmlASemmlSyntheticTenAllM+\SemmlASemmlSyntheticTenAllK/\SemmlASemmlSyntheticTenAllL]}
\newcommand{\SemmlASemmlSyntheticTenRealT}{1.7}
\newcommand{\SemmlASemmlSyntheticTenRealM}{22}
\newcommand{\SemmlASemmlSyntheticTenRealK}{2}
\newcommand{\SemmlASemmlSyntheticTenRealL}{10}
\newcommand{\SemmlASemmlSyntheticTenRealScore}{\SemmlASemmlSyntheticTenRealT[\SemmlASemmlSyntheticTenRealM+\SemmlASemmlSyntheticTenRealK/\SemmlASemmlSyntheticTenRealL]}
\newcommand{\SemmlASemmlSyntheticTenUnrealT}{1.26}
\newcommand{\SemmlASemmlSyntheticTenUnrealM}{34}
\newcommand{\SemmlASemmlSyntheticTenUnrealK}{2}
\newcommand{\SemmlASemmlSyntheticTenUnrealL}{10}
\newcommand{\SemmlASemmlSyntheticTenUnrealScore}{\SemmlASemmlSyntheticTenUnrealT[\SemmlASemmlSyntheticTenUnrealM+\SemmlASemmlSyntheticTenUnrealK/\SemmlASemmlSyntheticTenUnrealL]}
\newcommand{\StrixRealSyntcomptfTen}{98}
\newcommand{\StrixUnrealSyntcomptfTen}{62}
\newcommand{\SemmlARealSyntcomptfTen}{108}
\newcommand{\SemmlAUnrealSyntcomptfTen}{73}
\newcommand{\SemmlRealSyntcomptfTen}{110}
\newcommand{\SemmlUnrealSyntcomptfTen}{72}
\newcommand{\trivialSyntcomptfTen}{818}
\newcommand{\nontrivialSyntcomptfTen}{293}
\newcommand{\trivialStrixSemmlASyntcomptfTen}{825}
\newcommand{\unknownStrixSemmlASyntcomptfTen}{79}
\newcommand{\StrixSemmlASyntcomptfTenAllT}{1.71}
\newcommand{\StrixSemmlASyntcomptfTenAllM}{120}
\newcommand{\StrixSemmlASyntcomptfTenAllK}{33}
\newcommand{\StrixSemmlASyntcomptfTenAllL}{54}
\newcommand{\StrixSemmlASyntcomptfTenAllScore}{\StrixSemmlASyntcomptfTenAllT[\StrixSemmlASyntcomptfTenAllM+\StrixSemmlASyntcomptfTenAllK/\StrixSemmlASyntcomptfTenAllL]}
\newcommand{\StrixSemmlASyntcomptfTenRealT}{1.66}
\newcommand{\StrixSemmlASyntcomptfTenRealM}{83}
\newcommand{\StrixSemmlASyntcomptfTenRealK}{14}
\newcommand{\StrixSemmlASyntcomptfTenRealL}{24}
\newcommand{\StrixSemmlASyntcomptfTenRealScore}{\StrixSemmlASyntcomptfTenRealT[\StrixSemmlASyntcomptfTenRealM+\StrixSemmlASyntcomptfTenRealK/\StrixSemmlASyntcomptfTenRealL]}
\newcommand{\StrixSemmlASyntcomptfTenUnrealT}{1.85}
\newcommand{\StrixSemmlASyntcomptfTenUnrealM}{37}
\newcommand{\StrixSemmlASyntcomptfTenUnrealK}{19}
\newcommand{\StrixSemmlASyntcomptfTenUnrealL}{30}
\newcommand{\StrixSemmlASyntcomptfTenUnrealScore}{\StrixSemmlASyntcomptfTenUnrealT[\StrixSemmlASyntcomptfTenUnrealM+\StrixSemmlASyntcomptfTenUnrealK/\StrixSemmlASyntcomptfTenUnrealL]}
\newcommand{\trivialStrixSemmlSyntcomptfTen}{834}
\newcommand{\unknownStrixSemmlSyntcomptfTen}{84}
\newcommand{\StrixSemmlSyntcomptfTenAllT}{1.82}
\newcommand{\StrixSemmlSyntcomptfTenAllM}{117}
\newcommand{\StrixSemmlSyntcomptfTenAllK}{27}
\newcommand{\StrixSemmlSyntcomptfTenAllL}{49}
\newcommand{\StrixSemmlSyntcomptfTenAllScore}{\StrixSemmlSyntcomptfTenAllT[\StrixSemmlSyntcomptfTenAllM+\StrixSemmlSyntcomptfTenAllK/\StrixSemmlSyntcomptfTenAllL]}
\newcommand{\StrixSemmlSyntcomptfTenRealT}{2.11}
\newcommand{\StrixSemmlSyntcomptfTenRealM}{75}
\newcommand{\StrixSemmlSyntcomptfTenRealK}{12}
\newcommand{\StrixSemmlSyntcomptfTenRealL}{24}
\newcommand{\StrixSemmlSyntcomptfTenRealScore}{\StrixSemmlSyntcomptfTenRealT[\StrixSemmlSyntcomptfTenRealM+\StrixSemmlSyntcomptfTenRealK/\StrixSemmlSyntcomptfTenRealL]}
\newcommand{\StrixSemmlSyntcomptfTenUnrealT}{1.4}
\newcommand{\StrixSemmlSyntcomptfTenUnrealM}{42}
\newcommand{\StrixSemmlSyntcomptfTenUnrealK}{15}
\newcommand{\StrixSemmlSyntcomptfTenUnrealL}{25}
\newcommand{\StrixSemmlSyntcomptfTenUnrealScore}{\StrixSemmlSyntcomptfTenUnrealT[\StrixSemmlSyntcomptfTenUnrealM+\StrixSemmlSyntcomptfTenUnrealK/\StrixSemmlSyntcomptfTenUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcomptfTen}{835}
\newcommand{\unknownSemmlASemmlSyntcomptfTen}{102}
\newcommand{\SemmlASemmlSyntcomptfTenAllT}{0.93}
\newcommand{\SemmlASemmlSyntcomptfTenAllM}{155}
\newcommand{\SemmlASemmlSyntcomptfTenAllK}{9}
\newcommand{\SemmlASemmlSyntcomptfTenAllL}{10}
\newcommand{\SemmlASemmlSyntcomptfTenAllScore}{\SemmlASemmlSyntcomptfTenAllT[\SemmlASemmlSyntcomptfTenAllM+\SemmlASemmlSyntcomptfTenAllK/\SemmlASemmlSyntcomptfTenAllL]}
\newcommand{\SemmlASemmlSyntcomptfTenRealT}{1.05}
\newcommand{\SemmlASemmlSyntcomptfTenRealM}{95}
\newcommand{\SemmlASemmlSyntcomptfTenRealK}{1}
\newcommand{\SemmlASemmlSyntcomptfTenRealL}{3}
\newcommand{\SemmlASemmlSyntcomptfTenRealScore}{\SemmlASemmlSyntcomptfTenRealT[\SemmlASemmlSyntcomptfTenRealM+\SemmlASemmlSyntcomptfTenRealK/\SemmlASemmlSyntcomptfTenRealL]}
\newcommand{\SemmlASemmlSyntcomptfTenUnrealT}{0.77}
\newcommand{\SemmlASemmlSyntcomptfTenUnrealM}{60}
\newcommand{\SemmlASemmlSyntcomptfTenUnrealK}{8}
\newcommand{\SemmlASemmlSyntcomptfTenUnrealL}{7}
\newcommand{\SemmlASemmlSyntcomptfTenUnrealScore}{\SemmlASemmlSyntcomptfTenUnrealT[\SemmlASemmlSyntcomptfTenUnrealM+\SemmlASemmlSyntcomptfTenUnrealK/\SemmlASemmlSyntcomptfTenUnrealL]}
\newcommand{\StrixRealSyntcompThirty}{72}
\newcommand{\StrixUnrealSyntcompThirty}{50}
\newcommand{\SemmlARealSyntcompThirty}{82}
\newcommand{\SemmlAUnrealSyntcompThirty}{61}
\newcommand{\SemmlRealSyntcompThirty}{84}
\newcommand{\SemmlUnrealSyntcompThirty}{60}
\newcommand{\trivialSyntcompThirty}{821}
\newcommand{\nontrivialSyntcompThirty}{235}
\newcommand{\trivialStrixSemmlASyntcompThirty}{826}
\newcommand{\unknownStrixSemmlASyntcompThirty}{59}
\newcommand{\StrixSemmlASyntcompThirtyAllT}{1.8}
\newcommand{\StrixSemmlASyntcompThirtyAllM}{84}
\newcommand{\StrixSemmlASyntcompThirtyAllK}{33}
\newcommand{\StrixSemmlASyntcompThirtyAllL}{54}
\newcommand{\StrixSemmlASyntcompThirtyAllScore}{\StrixSemmlASyntcompThirtyAllT[\StrixSemmlASyntcompThirtyAllM+\StrixSemmlASyntcompThirtyAllK/\StrixSemmlASyntcompThirtyAllL]}
\newcommand{\StrixSemmlASyntcompThirtyRealT}{1.64}
\newcommand{\StrixSemmlASyntcompThirtyRealM}{58}
\newcommand{\StrixSemmlASyntcompThirtyRealK}{14}
\newcommand{\StrixSemmlASyntcompThirtyRealL}{24}
\newcommand{\StrixSemmlASyntcompThirtyRealScore}{\StrixSemmlASyntcompThirtyRealT[\StrixSemmlASyntcompThirtyRealM+\StrixSemmlASyntcompThirtyRealK/\StrixSemmlASyntcompThirtyRealL]}
\newcommand{\StrixSemmlASyntcompThirtyUnrealT}{2.22}
\newcommand{\StrixSemmlASyntcompThirtyUnrealM}{26}
\newcommand{\StrixSemmlASyntcompThirtyUnrealK}{19}
\newcommand{\StrixSemmlASyntcompThirtyUnrealL}{30}
\newcommand{\StrixSemmlASyntcompThirtyUnrealScore}{\StrixSemmlASyntcompThirtyUnrealT[\StrixSemmlASyntcompThirtyUnrealM+\StrixSemmlASyntcompThirtyUnrealK/\StrixSemmlASyntcompThirtyUnrealL]}
\newcommand{\trivialStrixSemmlSyntcompThirty}{837}
\newcommand{\unknownStrixSemmlSyntcompThirty}{64}
\newcommand{\StrixSemmlSyntcompThirtyAllT}{2.14}
\newcommand{\StrixSemmlSyntcompThirtyAllM}{79}
\newcommand{\StrixSemmlSyntcompThirtyAllK}{27}
\newcommand{\StrixSemmlSyntcompThirtyAllL}{49}
\newcommand{\StrixSemmlSyntcompThirtyAllScore}{\StrixSemmlSyntcompThirtyAllT[\StrixSemmlSyntcompThirtyAllM+\StrixSemmlSyntcompThirtyAllK/\StrixSemmlSyntcompThirtyAllL]}
\newcommand{\StrixSemmlSyntcompThirtyRealT}{2.54}
\newcommand{\StrixSemmlSyntcompThirtyRealM}{49}
\newcommand{\StrixSemmlSyntcompThirtyRealK}{12}
\newcommand{\StrixSemmlSyntcompThirtyRealL}{24}
\newcommand{\StrixSemmlSyntcompThirtyRealScore}{\StrixSemmlSyntcompThirtyRealT[\StrixSemmlSyntcompThirtyRealM+\StrixSemmlSyntcompThirtyRealK/\StrixSemmlSyntcompThirtyRealL]}
\newcommand{\StrixSemmlSyntcompThirtyUnrealT}{1.63}
\newcommand{\StrixSemmlSyntcompThirtyUnrealM}{30}
\newcommand{\StrixSemmlSyntcompThirtyUnrealK}{15}
\newcommand{\StrixSemmlSyntcompThirtyUnrealL}{25}
\newcommand{\StrixSemmlSyntcompThirtyUnrealScore}{\StrixSemmlSyntcompThirtyUnrealT[\StrixSemmlSyntcompThirtyUnrealM+\StrixSemmlSyntcompThirtyUnrealK/\StrixSemmlSyntcompThirtyUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcompThirty}{841}
\newcommand{\unknownSemmlASemmlSyntcompThirty}{82}
\newcommand{\SemmlASemmlSyntcompThirtyAllT}{1.02}
\newcommand{\SemmlASemmlSyntcompThirtyAllM}{114}
\newcommand{\SemmlASemmlSyntcompThirtyAllK}{9}
\newcommand{\SemmlASemmlSyntcompThirtyAllL}{10}
\newcommand{\SemmlASemmlSyntcompThirtyAllScore}{\SemmlASemmlSyntcompThirtyAllT[\SemmlASemmlSyntcompThirtyAllM+\SemmlASemmlSyntcompThirtyAllK/\SemmlASemmlSyntcompThirtyAllL]}
\newcommand{\SemmlASemmlSyntcompThirtyRealT}{1.25}
\newcommand{\SemmlASemmlSyntcompThirtyRealM}{66}
\newcommand{\SemmlASemmlSyntcompThirtyRealK}{1}
\newcommand{\SemmlASemmlSyntcompThirtyRealL}{3}
\newcommand{\SemmlASemmlSyntcompThirtyRealScore}{\SemmlASemmlSyntcompThirtyRealT[\SemmlASemmlSyntcompThirtyRealM+\SemmlASemmlSyntcompThirtyRealK/\SemmlASemmlSyntcompThirtyRealL]}
\newcommand{\SemmlASemmlSyntcompThirtyUnrealT}{0.76}
\newcommand{\SemmlASemmlSyntcompThirtyUnrealM}{48}
\newcommand{\SemmlASemmlSyntcompThirtyUnrealK}{8}
\newcommand{\SemmlASemmlSyntcompThirtyUnrealL}{7}
\newcommand{\SemmlASemmlSyntcompThirtyUnrealScore}{\SemmlASemmlSyntcompThirtyUnrealT[\SemmlASemmlSyntcompThirtyUnrealM+\SemmlASemmlSyntcompThirtyUnrealK/\SemmlASemmlSyntcompThirtyUnrealL]}
\newcommand{\StrixRealSyntheticThirty}{8}
\newcommand{\StrixUnrealSyntheticThirty}{20}
\newcommand{\SemmlARealSyntheticThirty}{27}
\newcommand{\SemmlAUnrealSyntheticThirty}{38}
\newcommand{\SemmlRealSyntheticThirty}{35}
\newcommand{\SemmlUnrealSyntheticThirty}{46}
\newcommand{\trivialSyntheticThirty}{2}
\newcommand{\nontrivialSyntheticThirty}{198}
\newcommand{\trivialStrixSemmlASyntheticThirty}{4}
\newcommand{\unknownStrixSemmlASyntheticThirty}{133}
\newcommand{\StrixSemmlASyntheticThirtyAllT}{10.08}
\newcommand{\StrixSemmlASyntheticThirtyAllM}{26}
\newcommand{\StrixSemmlASyntheticThirtyAllK}{0}
\newcommand{\StrixSemmlASyntheticThirtyAllL}{37}
\newcommand{\StrixSemmlASyntheticThirtyAllScore}{\StrixSemmlASyntheticThirtyAllT[\StrixSemmlASyntheticThirtyAllM+\StrixSemmlASyntheticThirtyAllK/\StrixSemmlASyntheticThirtyAllL]}
\newcommand{\StrixSemmlASyntheticThirtyRealT}{10.44}
\newcommand{\StrixSemmlASyntheticThirtyRealM}{8}
\newcommand{\StrixSemmlASyntheticThirtyRealK}{0}
\newcommand{\StrixSemmlASyntheticThirtyRealL}{19}
\newcommand{\StrixSemmlASyntheticThirtyRealScore}{\StrixSemmlASyntheticThirtyRealT[\StrixSemmlASyntheticThirtyRealM+\StrixSemmlASyntheticThirtyRealK/\StrixSemmlASyntheticThirtyRealL]}
\newcommand{\StrixSemmlASyntheticThirtyUnrealT}{9.92}
\newcommand{\StrixSemmlASyntheticThirtyUnrealM}{18}
\newcommand{\StrixSemmlASyntheticThirtyUnrealK}{0}
\newcommand{\StrixSemmlASyntheticThirtyUnrealL}{18}
\newcommand{\StrixSemmlASyntheticThirtyUnrealScore}{\StrixSemmlASyntheticThirtyUnrealT[\StrixSemmlASyntheticThirtyUnrealM+\StrixSemmlASyntheticThirtyUnrealK/\StrixSemmlASyntheticThirtyUnrealL]}
\newcommand{\trivialStrixSemmlSyntheticThirty}{2}
\newcommand{\unknownStrixSemmlSyntheticThirty}{117}
\newcommand{\StrixSemmlSyntheticThirtyAllT}{9.48}
\newcommand{\StrixSemmlSyntheticThirtyAllM}{28}
\newcommand{\StrixSemmlSyntheticThirtyAllK}{0}
\newcommand{\StrixSemmlSyntheticThirtyAllL}{53}
\newcommand{\StrixSemmlSyntheticThirtyAllScore}{\StrixSemmlSyntheticThirtyAllT[\StrixSemmlSyntheticThirtyAllM+\StrixSemmlSyntheticThirtyAllK/\StrixSemmlSyntheticThirtyAllL]}
\newcommand{\StrixSemmlSyntheticThirtyRealT}{13.07}
\newcommand{\StrixSemmlSyntheticThirtyRealM}{8}
\newcommand{\StrixSemmlSyntheticThirtyRealK}{0}
\newcommand{\StrixSemmlSyntheticThirtyRealL}{27}
\newcommand{\StrixSemmlSyntheticThirtyRealScore}{\StrixSemmlSyntheticThirtyRealT[\StrixSemmlSyntheticThirtyRealM+\StrixSemmlSyntheticThirtyRealK/\StrixSemmlSyntheticThirtyRealL]}
\newcommand{\StrixSemmlSyntheticThirtyUnrealT}{8.34}
\newcommand{\StrixSemmlSyntheticThirtyUnrealM}{20}
\newcommand{\StrixSemmlSyntheticThirtyUnrealK}{0}
\newcommand{\StrixSemmlSyntheticThirtyUnrealL}{26}
\newcommand{\StrixSemmlSyntheticThirtyUnrealScore}{\StrixSemmlSyntheticThirtyUnrealT[\StrixSemmlSyntheticThirtyUnrealM+\StrixSemmlSyntheticThirtyUnrealK/\StrixSemmlSyntheticThirtyUnrealL]}
\newcommand{\trivialSemmlASemmlSyntheticThirty}{18}
\newcommand{\unknownSemmlASemmlSyntheticThirty}{113}
\newcommand{\SemmlASemmlSyntheticThirtyAllT}{1.57}
\newcommand{\SemmlASemmlSyntheticThirtyAllM}{45}
\newcommand{\SemmlASemmlSyntheticThirtyAllK}{4}
\newcommand{\SemmlASemmlSyntheticThirtyAllL}{20}
\newcommand{\SemmlASemmlSyntheticThirtyAllScore}{\SemmlASemmlSyntheticThirtyAllT[\SemmlASemmlSyntheticThirtyAllM+\SemmlASemmlSyntheticThirtyAllK/\SemmlASemmlSyntheticThirtyAllL]}
\newcommand{\SemmlASemmlSyntheticThirtyRealT}{1.95}
\newcommand{\SemmlASemmlSyntheticThirtyRealM}{16}
\newcommand{\SemmlASemmlSyntheticThirtyRealK}{2}
\newcommand{\SemmlASemmlSyntheticThirtyRealL}{10}
\newcommand{\SemmlASemmlSyntheticThirtyRealScore}{\SemmlASemmlSyntheticThirtyRealT[\SemmlASemmlSyntheticThirtyRealM+\SemmlASemmlSyntheticThirtyRealK/\SemmlASemmlSyntheticThirtyRealL]}
\newcommand{\SemmlASemmlSyntheticThirtyUnrealT}{1.39}
\newcommand{\SemmlASemmlSyntheticThirtyUnrealM}{29}
\newcommand{\SemmlASemmlSyntheticThirtyUnrealK}{2}
\newcommand{\SemmlASemmlSyntheticThirtyUnrealL}{10}
\newcommand{\SemmlASemmlSyntheticThirtyUnrealScore}{\SemmlASemmlSyntheticThirtyUnrealT[\SemmlASemmlSyntheticThirtyUnrealM+\SemmlASemmlSyntheticThirtyUnrealK/\SemmlASemmlSyntheticThirtyUnrealL]}
\newcommand{\StrixRealSyntcomptfThirty}{81}
\newcommand{\StrixUnrealSyntcomptfThirty}{51}
\newcommand{\SemmlARealSyntcomptfThirty}{91}
\newcommand{\SemmlAUnrealSyntcomptfThirty}{62}
\newcommand{\SemmlRealSyntcomptfThirty}{93}
\newcommand{\SemmlUnrealSyntcomptfThirty}{61}
\newcommand{\trivialSyntcomptfThirty}{846}
\newcommand{\nontrivialSyntcomptfThirty}{265}
\newcommand{\trivialStrixSemmlASyntcomptfThirty}{851}
\newcommand{\unknownStrixSemmlASyntcomptfThirty}{79}
\newcommand{\StrixSemmlASyntcomptfThirtyAllT}{1.8}
\newcommand{\StrixSemmlASyntcomptfThirtyAllM}{94}
\newcommand{\StrixSemmlASyntcomptfThirtyAllK}{33}
\newcommand{\StrixSemmlASyntcomptfThirtyAllL}{54}
\newcommand{\StrixSemmlASyntcomptfThirtyAllScore}{\StrixSemmlASyntcomptfThirtyAllT[\StrixSemmlASyntcomptfThirtyAllM+\StrixSemmlASyntcomptfThirtyAllK/\StrixSemmlASyntcomptfThirtyAllL]}
\newcommand{\StrixSemmlASyntcomptfThirtyRealT}{1.65}
\newcommand{\StrixSemmlASyntcomptfThirtyRealM}{67}
\newcommand{\StrixSemmlASyntcomptfThirtyRealK}{14}
\newcommand{\StrixSemmlASyntcomptfThirtyRealL}{24}
\newcommand{\StrixSemmlASyntcomptfThirtyRealScore}{\StrixSemmlASyntcomptfThirtyRealT[\StrixSemmlASyntcomptfThirtyRealM+\StrixSemmlASyntcomptfThirtyRealK/\StrixSemmlASyntcomptfThirtyRealL]}
\newcommand{\StrixSemmlASyntcomptfThirtyUnrealT}{2.24}
\newcommand{\StrixSemmlASyntcomptfThirtyUnrealM}{27}
\newcommand{\StrixSemmlASyntcomptfThirtyUnrealK}{19}
\newcommand{\StrixSemmlASyntcomptfThirtyUnrealL}{30}
\newcommand{\StrixSemmlASyntcomptfThirtyUnrealScore}{\StrixSemmlASyntcomptfThirtyUnrealT[\StrixSemmlASyntcomptfThirtyUnrealM+\StrixSemmlASyntcomptfThirtyUnrealK/\StrixSemmlASyntcomptfThirtyUnrealL]}
\newcommand{\trivialStrixSemmlSyntcomptfThirty}{862}
\newcommand{\unknownStrixSemmlSyntcomptfThirty}{84}
\newcommand{\StrixSemmlSyntcomptfThirtyAllT}{2.08}
\newcommand{\StrixSemmlSyntcomptfThirtyAllM}{89}
\newcommand{\StrixSemmlSyntcomptfThirtyAllK}{27}
\newcommand{\StrixSemmlSyntcomptfThirtyAllL}{49}
\newcommand{\StrixSemmlSyntcomptfThirtyAllScore}{\StrixSemmlSyntcomptfThirtyAllT[\StrixSemmlSyntcomptfThirtyAllM+\StrixSemmlSyntcomptfThirtyAllK/\StrixSemmlSyntcomptfThirtyAllL]}
\newcommand{\StrixSemmlSyntcomptfThirtyRealT}{2.35}
\newcommand{\StrixSemmlSyntcomptfThirtyRealM}{58}
\newcommand{\StrixSemmlSyntcomptfThirtyRealK}{12}
\newcommand{\StrixSemmlSyntcomptfThirtyRealL}{24}
\newcommand{\StrixSemmlSyntcomptfThirtyRealScore}{\StrixSemmlSyntcomptfThirtyRealT[\StrixSemmlSyntcomptfThirtyRealM+\StrixSemmlSyntcomptfThirtyRealK/\StrixSemmlSyntcomptfThirtyRealL]}
\newcommand{\StrixSemmlSyntcomptfThirtyUnrealT}{1.65}
\newcommand{\StrixSemmlSyntcomptfThirtyUnrealM}{31}
\newcommand{\StrixSemmlSyntcomptfThirtyUnrealK}{15}
\newcommand{\StrixSemmlSyntcomptfThirtyUnrealL}{25}
\newcommand{\StrixSemmlSyntcomptfThirtyUnrealScore}{\StrixSemmlSyntcomptfThirtyUnrealT[\StrixSemmlSyntcomptfThirtyUnrealM+\StrixSemmlSyntcomptfThirtyUnrealK/\StrixSemmlSyntcomptfThirtyUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcomptfThirty}{867}
\newcommand{\unknownSemmlASemmlSyntcomptfThirty}{102}
\newcommand{\SemmlASemmlSyntcomptfThirtyAllT}{1.01}
\newcommand{\SemmlASemmlSyntcomptfThirtyAllM}{123}
\newcommand{\SemmlASemmlSyntcomptfThirtyAllK}{9}
\newcommand{\SemmlASemmlSyntcomptfThirtyAllL}{10}
\newcommand{\SemmlASemmlSyntcomptfThirtyAllScore}{\SemmlASemmlSyntcomptfThirtyAllT[\SemmlASemmlSyntcomptfThirtyAllM+\SemmlASemmlSyntcomptfThirtyAllK/\SemmlASemmlSyntcomptfThirtyAllL]}
\newcommand{\SemmlASemmlSyntcomptfThirtyRealT}{1.21}
\newcommand{\SemmlASemmlSyntcomptfThirtyRealM}{74}
\newcommand{\SemmlASemmlSyntcomptfThirtyRealK}{1}
\newcommand{\SemmlASemmlSyntcomptfThirtyRealL}{3}
\newcommand{\SemmlASemmlSyntcomptfThirtyRealScore}{\SemmlASemmlSyntcomptfThirtyRealT[\SemmlASemmlSyntcomptfThirtyRealM+\SemmlASemmlSyntcomptfThirtyRealK/\SemmlASemmlSyntcomptfThirtyRealL]}
\newcommand{\SemmlASemmlSyntcomptfThirtyUnrealT}{0.77}
\newcommand{\SemmlASemmlSyntcomptfThirtyUnrealM}{49}
\newcommand{\SemmlASemmlSyntcomptfThirtyUnrealK}{8}
\newcommand{\SemmlASemmlSyntcomptfThirtyUnrealL}{7}
\newcommand{\SemmlASemmlSyntcomptfThirtyUnrealScore}{\SemmlASemmlSyntcomptfThirtyUnrealT[\SemmlASemmlSyntcomptfThirtyUnrealM+\SemmlASemmlSyntcomptfThirtyUnrealK/\SemmlASemmlSyntcomptfThirtyUnrealL]}
\newcommand{\StrixRealSyntcompSixty}{56}
\newcommand{\StrixUnrealSyntcompSixty}{42}
\newcommand{\SemmlARealSyntcompSixty}{66}
\newcommand{\SemmlAUnrealSyntcompSixty}{53}
\newcommand{\SemmlRealSyntcompSixty}{68}
\newcommand{\SemmlUnrealSyntcompSixty}{52}
\newcommand{\trivialSyntcompSixty}{845}
\newcommand{\nontrivialSyntcompSixty}{211}
\newcommand{\trivialStrixSemmlASyntcompSixty}{846}
\newcommand{\unknownStrixSemmlASyntcompSixty}{59}
\newcommand{\StrixSemmlASyntcompSixtyAllT}{2.66}
\newcommand{\StrixSemmlASyntcompSixtyAllM}{64}
\newcommand{\StrixSemmlASyntcompSixtyAllK}{33}
\newcommand{\StrixSemmlASyntcompSixtyAllL}{54}
\newcommand{\StrixSemmlASyntcompSixtyAllScore}{\StrixSemmlASyntcompSixtyAllT[\StrixSemmlASyntcompSixtyAllM+\StrixSemmlASyntcompSixtyAllK/\StrixSemmlASyntcompSixtyAllL]}
\newcommand{\StrixSemmlASyntcompSixtyRealT}{2.83}
\newcommand{\StrixSemmlASyntcompSixtyRealM}{42}
\newcommand{\StrixSemmlASyntcompSixtyRealK}{14}
\newcommand{\StrixSemmlASyntcompSixtyRealL}{24}
\newcommand{\StrixSemmlASyntcompSixtyRealScore}{\StrixSemmlASyntcompSixtyRealT[\StrixSemmlASyntcompSixtyRealM+\StrixSemmlASyntcompSixtyRealK/\StrixSemmlASyntcompSixtyRealL]}
\newcommand{\StrixSemmlASyntcompSixtyUnrealT}{2.36}
\newcommand{\StrixSemmlASyntcompSixtyUnrealM}{22}
\newcommand{\StrixSemmlASyntcompSixtyUnrealK}{19}
\newcommand{\StrixSemmlASyntcompSixtyUnrealL}{30}
\newcommand{\StrixSemmlASyntcompSixtyUnrealScore}{\StrixSemmlASyntcompSixtyUnrealT[\StrixSemmlASyntcompSixtyUnrealM+\StrixSemmlASyntcompSixtyUnrealK/\StrixSemmlASyntcompSixtyUnrealL]}
\newcommand{\trivialStrixSemmlSyntcompSixty}{855}
\newcommand{\unknownStrixSemmlSyntcompSixty}{64}
\newcommand{\StrixSemmlSyntcompSixtyAllT}{2.71}
\newcommand{\StrixSemmlSyntcompSixtyAllM}{61}
\newcommand{\StrixSemmlSyntcompSixtyAllK}{27}
\newcommand{\StrixSemmlSyntcompSixtyAllL}{49}
\newcommand{\StrixSemmlSyntcompSixtyAllScore}{\StrixSemmlSyntcompSixtyAllT[\StrixSemmlSyntcompSixtyAllM+\StrixSemmlSyntcompSixtyAllK/\StrixSemmlSyntcompSixtyAllL]}
\newcommand{\StrixSemmlSyntcompSixtyRealT}{2.85}
\newcommand{\StrixSemmlSyntcompSixtyRealM}{40}
\newcommand{\StrixSemmlSyntcompSixtyRealK}{12}
\newcommand{\StrixSemmlSyntcompSixtyRealL}{24}
\newcommand{\StrixSemmlSyntcompSixtyRealScore}{\StrixSemmlSyntcompSixtyRealT[\StrixSemmlSyntcompSixtyRealM+\StrixSemmlSyntcompSixtyRealK/\StrixSemmlSyntcompSixtyRealL]}
\newcommand{\StrixSemmlSyntcompSixtyUnrealT}{2.47}
\newcommand{\StrixSemmlSyntcompSixtyUnrealM}{21}
\newcommand{\StrixSemmlSyntcompSixtyUnrealK}{15}
\newcommand{\StrixSemmlSyntcompSixtyUnrealL}{25}
\newcommand{\StrixSemmlSyntcompSixtyUnrealScore}{\StrixSemmlSyntcompSixtyUnrealT[\StrixSemmlSyntcompSixtyUnrealM+\StrixSemmlSyntcompSixtyUnrealK/\StrixSemmlSyntcompSixtyUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcompSixty}{867}
\newcommand{\unknownSemmlASemmlSyntcompSixty}{82}
\newcommand{\SemmlASemmlSyntcompSixtyAllT}{0.95}
\newcommand{\SemmlASemmlSyntcompSixtyAllM}{88}
\newcommand{\SemmlASemmlSyntcompSixtyAllK}{9}
\newcommand{\SemmlASemmlSyntcompSixtyAllL}{10}
\newcommand{\SemmlASemmlSyntcompSixtyAllScore}{\SemmlASemmlSyntcompSixtyAllT[\SemmlASemmlSyntcompSixtyAllM+\SemmlASemmlSyntcompSixtyAllK/\SemmlASemmlSyntcompSixtyAllL]}
\newcommand{\SemmlASemmlSyntcompSixtyRealT}{1.02}
\newcommand{\SemmlASemmlSyntcompSixtyRealM}{51}
\newcommand{\SemmlASemmlSyntcompSixtyRealK}{1}
\newcommand{\SemmlASemmlSyntcompSixtyRealL}{3}
\newcommand{\SemmlASemmlSyntcompSixtyRealScore}{\SemmlASemmlSyntcompSixtyRealT[\SemmlASemmlSyntcompSixtyRealM+\SemmlASemmlSyntcompSixtyRealK/\SemmlASemmlSyntcompSixtyRealL]}
\newcommand{\SemmlASemmlSyntcompSixtyUnrealT}{0.87}
\newcommand{\SemmlASemmlSyntcompSixtyUnrealM}{37}
\newcommand{\SemmlASemmlSyntcompSixtyUnrealK}{8}
\newcommand{\SemmlASemmlSyntcompSixtyUnrealL}{7}
\newcommand{\SemmlASemmlSyntcompSixtyUnrealScore}{\SemmlASemmlSyntcompSixtyUnrealT[\SemmlASemmlSyntcompSixtyUnrealM+\SemmlASemmlSyntcompSixtyUnrealK/\SemmlASemmlSyntcompSixtyUnrealL]}
\newcommand{\StrixRealSyntheticSixty}{7}
\newcommand{\StrixUnrealSyntheticSixty}{17}
\newcommand{\SemmlARealSyntheticSixty}{26}
\newcommand{\SemmlAUnrealSyntheticSixty}{35}
\newcommand{\SemmlRealSyntheticSixty}{34}
\newcommand{\SemmlUnrealSyntheticSixty}{43}
\newcommand{\trivialSyntheticSixty}{6}
\newcommand{\nontrivialSyntheticSixty}{194}
\newcommand{\trivialStrixSemmlASyntheticSixty}{6}
\newcommand{\unknownStrixSemmlASyntheticSixty}{133}
\newcommand{\StrixSemmlASyntheticSixtyAllT}{10.71}
\newcommand{\StrixSemmlASyntheticSixtyAllM}{24}
\newcommand{\StrixSemmlASyntheticSixtyAllK}{0}
\newcommand{\StrixSemmlASyntheticSixtyAllL}{37}
\newcommand{\StrixSemmlASyntheticSixtyAllScore}{\StrixSemmlASyntheticSixtyAllT[\StrixSemmlASyntheticSixtyAllM+\StrixSemmlASyntheticSixtyAllK/\StrixSemmlASyntheticSixtyAllL]}
\newcommand{\StrixSemmlASyntheticSixtyRealT}{13.09}
\newcommand{\StrixSemmlASyntheticSixtyRealM}{7}
\newcommand{\StrixSemmlASyntheticSixtyRealK}{0}
\newcommand{\StrixSemmlASyntheticSixtyRealL}{19}
\newcommand{\StrixSemmlASyntheticSixtyRealScore}{\StrixSemmlASyntheticSixtyRealT[\StrixSemmlASyntheticSixtyRealM+\StrixSemmlASyntheticSixtyRealK/\StrixSemmlASyntheticSixtyRealL]}
\newcommand{\StrixSemmlASyntheticSixtyUnrealT}{9.86}
\newcommand{\StrixSemmlASyntheticSixtyUnrealM}{17}
\newcommand{\StrixSemmlASyntheticSixtyUnrealK}{0}
\newcommand{\StrixSemmlASyntheticSixtyUnrealL}{18}
\newcommand{\StrixSemmlASyntheticSixtyUnrealScore}{\StrixSemmlASyntheticSixtyUnrealT[\StrixSemmlASyntheticSixtyUnrealM+\StrixSemmlASyntheticSixtyUnrealK/\StrixSemmlASyntheticSixtyUnrealL]}
\newcommand{\trivialStrixSemmlSyntheticSixty}{6}
\newcommand{\unknownStrixSemmlSyntheticSixty}{117}
\newcommand{\StrixSemmlSyntheticSixtyAllT}{13.16}
\newcommand{\StrixSemmlSyntheticSixtyAllM}{24}
\newcommand{\StrixSemmlSyntheticSixtyAllK}{0}
\newcommand{\StrixSemmlSyntheticSixtyAllL}{53}
\newcommand{\StrixSemmlSyntheticSixtyAllScore}{\StrixSemmlSyntheticSixtyAllT[\StrixSemmlSyntheticSixtyAllM+\StrixSemmlSyntheticSixtyAllK/\StrixSemmlSyntheticSixtyAllL]}
\newcommand{\StrixSemmlSyntheticSixtyRealT}{16.3}
\newcommand{\StrixSemmlSyntheticSixtyRealM}{7}
\newcommand{\StrixSemmlSyntheticSixtyRealK}{0}
\newcommand{\StrixSemmlSyntheticSixtyRealL}{27}
\newcommand{\StrixSemmlSyntheticSixtyRealScore}{\StrixSemmlSyntheticSixtyRealT[\StrixSemmlSyntheticSixtyRealM+\StrixSemmlSyntheticSixtyRealK/\StrixSemmlSyntheticSixtyRealL]}
\newcommand{\StrixSemmlSyntheticSixtyUnrealT}{12.05}
\newcommand{\StrixSemmlSyntheticSixtyUnrealM}{17}
\newcommand{\StrixSemmlSyntheticSixtyUnrealK}{0}
\newcommand{\StrixSemmlSyntheticSixtyUnrealL}{26}
\newcommand{\StrixSemmlSyntheticSixtyUnrealScore}{\StrixSemmlSyntheticSixtyUnrealT[\StrixSemmlSyntheticSixtyUnrealM+\StrixSemmlSyntheticSixtyUnrealK/\StrixSemmlSyntheticSixtyUnrealL]}
\newcommand{\trivialSemmlASemmlSyntheticSixty}{29}
\newcommand{\unknownSemmlASemmlSyntheticSixty}{113}
\newcommand{\SemmlASemmlSyntheticSixtyAllT}{1.89}
\newcommand{\SemmlASemmlSyntheticSixtyAllM}{34}
\newcommand{\SemmlASemmlSyntheticSixtyAllK}{4}
\newcommand{\SemmlASemmlSyntheticSixtyAllL}{20}
\newcommand{\SemmlASemmlSyntheticSixtyAllScore}{\SemmlASemmlSyntheticSixtyAllT[\SemmlASemmlSyntheticSixtyAllM+\SemmlASemmlSyntheticSixtyAllK/\SemmlASemmlSyntheticSixtyAllL]}
\newcommand{\SemmlASemmlSyntheticSixtyRealT}{2.19}
\newcommand{\SemmlASemmlSyntheticSixtyRealM}{14}
\newcommand{\SemmlASemmlSyntheticSixtyRealK}{2}
\newcommand{\SemmlASemmlSyntheticSixtyRealL}{10}
\newcommand{\SemmlASemmlSyntheticSixtyRealScore}{\SemmlASemmlSyntheticSixtyRealT[\SemmlASemmlSyntheticSixtyRealM+\SemmlASemmlSyntheticSixtyRealK/\SemmlASemmlSyntheticSixtyRealL]}
\newcommand{\SemmlASemmlSyntheticSixtyUnrealT}{1.7}
\newcommand{\SemmlASemmlSyntheticSixtyUnrealM}{20}
\newcommand{\SemmlASemmlSyntheticSixtyUnrealK}{2}
\newcommand{\SemmlASemmlSyntheticSixtyUnrealL}{10}
\newcommand{\SemmlASemmlSyntheticSixtyUnrealScore}{\SemmlASemmlSyntheticSixtyUnrealT[\SemmlASemmlSyntheticSixtyUnrealM+\SemmlASemmlSyntheticSixtyUnrealK/\SemmlASemmlSyntheticSixtyUnrealL]}
\newcommand{\StrixRealSyntcomptfSixty}{65}
\newcommand{\StrixUnrealSyntcomptfSixty}{43}
\newcommand{\SemmlARealSyntcomptfSixty}{75}
\newcommand{\SemmlAUnrealSyntcomptfSixty}{54}
\newcommand{\SemmlRealSyntcomptfSixty}{77}
\newcommand{\SemmlUnrealSyntcomptfSixty}{53}
\newcommand{\trivialSyntcomptfSixty}{870}
\newcommand{\nontrivialSyntcomptfSixty}{241}
\newcommand{\trivialStrixSemmlASyntcomptfSixty}{871}
\newcommand{\unknownStrixSemmlASyntcomptfSixty}{79}
\newcommand{\StrixSemmlASyntcomptfSixtyAllT}{2.53}
\newcommand{\StrixSemmlASyntcomptfSixtyAllM}{74}
\newcommand{\StrixSemmlASyntcomptfSixtyAllK}{33}
\newcommand{\StrixSemmlASyntcomptfSixtyAllL}{54}
\newcommand{\StrixSemmlASyntcomptfSixtyAllScore}{\StrixSemmlASyntcomptfSixtyAllT[\StrixSemmlASyntcomptfSixtyAllM+\StrixSemmlASyntcomptfSixtyAllK/\StrixSemmlASyntcomptfSixtyAllL]}
\newcommand{\StrixSemmlASyntcomptfSixtyRealT}{2.6}
\newcommand{\StrixSemmlASyntcomptfSixtyRealM}{51}
\newcommand{\StrixSemmlASyntcomptfSixtyRealK}{14}
\newcommand{\StrixSemmlASyntcomptfSixtyRealL}{24}
\newcommand{\StrixSemmlASyntcomptfSixtyRealScore}{\StrixSemmlASyntcomptfSixtyRealT[\StrixSemmlASyntcomptfSixtyRealM+\StrixSemmlASyntcomptfSixtyRealK/\StrixSemmlASyntcomptfSixtyRealL]}
\newcommand{\StrixSemmlASyntcomptfSixtyUnrealT}{2.38}
\newcommand{\StrixSemmlASyntcomptfSixtyUnrealM}{23}
\newcommand{\StrixSemmlASyntcomptfSixtyUnrealK}{19}
\newcommand{\StrixSemmlASyntcomptfSixtyUnrealL}{30}
\newcommand{\StrixSemmlASyntcomptfSixtyUnrealScore}{\StrixSemmlASyntcomptfSixtyUnrealT[\StrixSemmlASyntcomptfSixtyUnrealM+\StrixSemmlASyntcomptfSixtyUnrealK/\StrixSemmlASyntcomptfSixtyUnrealL]}
\newcommand{\trivialStrixSemmlSyntcomptfSixty}{880}
\newcommand{\unknownStrixSemmlSyntcomptfSixty}{84}
\newcommand{\StrixSemmlSyntcomptfSixtyAllT}{2.52}
\newcommand{\StrixSemmlSyntcomptfSixtyAllM}{71}
\newcommand{\StrixSemmlSyntcomptfSixtyAllK}{27}
\newcommand{\StrixSemmlSyntcomptfSixtyAllL}{49}
\newcommand{\StrixSemmlSyntcomptfSixtyAllScore}{\StrixSemmlSyntcomptfSixtyAllT[\StrixSemmlSyntcomptfSixtyAllM+\StrixSemmlSyntcomptfSixtyAllK/\StrixSemmlSyntcomptfSixtyAllL]}
\newcommand{\StrixSemmlSyntcomptfSixtyRealT}{2.55}
\newcommand{\StrixSemmlSyntcomptfSixtyRealM}{49}
\newcommand{\StrixSemmlSyntcomptfSixtyRealK}{12}
\newcommand{\StrixSemmlSyntcomptfSixtyRealL}{24}
\newcommand{\StrixSemmlSyntcomptfSixtyRealScore}{\StrixSemmlSyntcomptfSixtyRealT[\StrixSemmlSyntcomptfSixtyRealM+\StrixSemmlSyntcomptfSixtyRealK/\StrixSemmlSyntcomptfSixtyRealL]}
\newcommand{\StrixSemmlSyntcomptfSixtyUnrealT}{2.47}
\newcommand{\StrixSemmlSyntcomptfSixtyUnrealM}{22}
\newcommand{\StrixSemmlSyntcomptfSixtyUnrealK}{15}
\newcommand{\StrixSemmlSyntcomptfSixtyUnrealL}{25}
\newcommand{\StrixSemmlSyntcomptfSixtyUnrealScore}{\StrixSemmlSyntcomptfSixtyUnrealT[\StrixSemmlSyntcomptfSixtyUnrealM+\StrixSemmlSyntcomptfSixtyUnrealK/\StrixSemmlSyntcomptfSixtyUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcomptfSixty}{897}
\newcommand{\unknownSemmlASemmlSyntcomptfSixty}{102}
\newcommand{\SemmlASemmlSyntcomptfSixtyAllT}{0.95}
\newcommand{\SemmlASemmlSyntcomptfSixtyAllM}{93}
\newcommand{\SemmlASemmlSyntcomptfSixtyAllK}{9}
\newcommand{\SemmlASemmlSyntcomptfSixtyAllL}{10}
\newcommand{\SemmlASemmlSyntcomptfSixtyAllScore}{\SemmlASemmlSyntcomptfSixtyAllT[\SemmlASemmlSyntcomptfSixtyAllM+\SemmlASemmlSyntcomptfSixtyAllK/\SemmlASemmlSyntcomptfSixtyAllL]}
\newcommand{\SemmlASemmlSyntcomptfSixtyRealT}{1.01}
\newcommand{\SemmlASemmlSyntcomptfSixtyRealM}{56}
\newcommand{\SemmlASemmlSyntcomptfSixtyRealK}{1}
\newcommand{\SemmlASemmlSyntcomptfSixtyRealL}{3}
\newcommand{\SemmlASemmlSyntcomptfSixtyRealScore}{\SemmlASemmlSyntcomptfSixtyRealT[\SemmlASemmlSyntcomptfSixtyRealM+\SemmlASemmlSyntcomptfSixtyRealK/\SemmlASemmlSyntcomptfSixtyRealL]}
\newcommand{\SemmlASemmlSyntcomptfSixtyUnrealT}{0.87}
\newcommand{\SemmlASemmlSyntcomptfSixtyUnrealM}{37}
\newcommand{\SemmlASemmlSyntcomptfSixtyUnrealK}{8}
\newcommand{\SemmlASemmlSyntcomptfSixtyUnrealL}{7}
\newcommand{\SemmlASemmlSyntcomptfSixtyUnrealScore}{\SemmlASemmlSyntcomptfSixtyUnrealT[\SemmlASemmlSyntcomptfSixtyUnrealM+\SemmlASemmlSyntcomptfSixtyUnrealK/\SemmlASemmlSyntcomptfSixtyUnrealL]}
\newcommand{\StrixRealSyntcompThreehundred}{35}
\newcommand{\StrixUnrealSyntcompThreehundred}{27}
\newcommand{\SemmlARealSyntcompThreehundred}{45}
\newcommand{\SemmlAUnrealSyntcompThreehundred}{38}
\newcommand{\SemmlRealSyntcompThreehundred}{47}
\newcommand{\SemmlUnrealSyntcompThreehundred}{37}
\newcommand{\trivialSyntcompThreehundred}{881}
\newcommand{\nontrivialSyntcompThreehundred}{175}
\newcommand{\trivialStrixSemmlASyntcompThreehundred}{881}
\newcommand{\unknownStrixSemmlASyntcompThreehundred}{59}
\newcommand{\StrixSemmlASyntcompThreehundredAllT}{3.68}
\newcommand{\StrixSemmlASyntcompThreehundredAllM}{29}
\newcommand{\StrixSemmlASyntcompThreehundredAllK}{33}
\newcommand{\StrixSemmlASyntcompThreehundredAllL}{54}
\newcommand{\StrixSemmlASyntcompThreehundredAllScore}{\StrixSemmlASyntcompThreehundredAllT[\StrixSemmlASyntcompThreehundredAllM+\StrixSemmlASyntcompThreehundredAllK/\StrixSemmlASyntcompThreehundredAllL]}
\newcommand{\StrixSemmlASyntcompThreehundredRealT}{4.61}
\newcommand{\StrixSemmlASyntcompThreehundredRealM}{21}
\newcommand{\StrixSemmlASyntcompThreehundredRealK}{14}
\newcommand{\StrixSemmlASyntcompThreehundredRealL}{24}
\newcommand{\StrixSemmlASyntcompThreehundredRealScore}{\StrixSemmlASyntcompThreehundredRealT[\StrixSemmlASyntcompThreehundredRealM+\StrixSemmlASyntcompThreehundredRealK/\StrixSemmlASyntcompThreehundredRealL]}
\newcommand{\StrixSemmlASyntcompThreehundredUnrealT}{2.03}
\newcommand{\StrixSemmlASyntcompThreehundredUnrealM}{8}
\newcommand{\StrixSemmlASyntcompThreehundredUnrealK}{19}
\newcommand{\StrixSemmlASyntcompThreehundredUnrealL}{30}
\newcommand{\StrixSemmlASyntcompThreehundredUnrealScore}{\StrixSemmlASyntcompThreehundredUnrealT[\StrixSemmlASyntcompThreehundredUnrealM+\StrixSemmlASyntcompThreehundredUnrealK/\StrixSemmlASyntcompThreehundredUnrealL]}
\newcommand{\trivialStrixSemmlSyntcompThreehundred}{890}
\newcommand{\unknownStrixSemmlSyntcompThreehundred}{64}
\newcommand{\StrixSemmlSyntcompThreehundredAllT}{4.19}
\newcommand{\StrixSemmlSyntcompThreehundredAllM}{26}
\newcommand{\StrixSemmlSyntcompThreehundredAllK}{27}
\newcommand{\StrixSemmlSyntcompThreehundredAllL}{49}
\newcommand{\StrixSemmlSyntcompThreehundredAllScore}{\StrixSemmlSyntcompThreehundredAllT[\StrixSemmlSyntcompThreehundredAllM+\StrixSemmlSyntcompThreehundredAllK/\StrixSemmlSyntcompThreehundredAllL]}
\newcommand{\StrixSemmlSyntcompThreehundredRealT}{3.75}
\newcommand{\StrixSemmlSyntcompThreehundredRealM}{20}
\newcommand{\StrixSemmlSyntcompThreehundredRealK}{12}
\newcommand{\StrixSemmlSyntcompThreehundredRealL}{24}
\newcommand{\StrixSemmlSyntcompThreehundredRealScore}{\StrixSemmlSyntcompThreehundredRealT[\StrixSemmlSyntcompThreehundredRealM+\StrixSemmlSyntcompThreehundredRealK/\StrixSemmlSyntcompThreehundredRealL]}
\newcommand{\StrixSemmlSyntcompThreehundredUnrealT}{6.06}
\newcommand{\StrixSemmlSyntcompThreehundredUnrealM}{6}
\newcommand{\StrixSemmlSyntcompThreehundredUnrealK}{15}
\newcommand{\StrixSemmlSyntcompThreehundredUnrealL}{25}
\newcommand{\StrixSemmlSyntcompThreehundredUnrealScore}{\StrixSemmlSyntcompThreehundredUnrealT[\StrixSemmlSyntcompThreehundredUnrealM+\StrixSemmlSyntcompThreehundredUnrealK/\StrixSemmlSyntcompThreehundredUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcompThreehundred}{919}
\newcommand{\unknownSemmlASemmlSyntcompThreehundred}{82}
\newcommand{\SemmlASemmlSyntcompThreehundredAllT}{0.98}
\newcommand{\SemmlASemmlSyntcompThreehundredAllM}{36}
\newcommand{\SemmlASemmlSyntcompThreehundredAllK}{9}
\newcommand{\SemmlASemmlSyntcompThreehundredAllL}{10}
\newcommand{\SemmlASemmlSyntcompThreehundredAllScore}{\SemmlASemmlSyntcompThreehundredAllT[\SemmlASemmlSyntcompThreehundredAllM+\SemmlASemmlSyntcompThreehundredAllK/\SemmlASemmlSyntcompThreehundredAllL]}
\newcommand{\SemmlASemmlSyntcompThreehundredRealT}{0.9}
\newcommand{\SemmlASemmlSyntcompThreehundredRealM}{22}
\newcommand{\SemmlASemmlSyntcompThreehundredRealK}{1}
\newcommand{\SemmlASemmlSyntcompThreehundredRealL}{3}
\newcommand{\SemmlASemmlSyntcompThreehundredRealScore}{\SemmlASemmlSyntcompThreehundredRealT[\SemmlASemmlSyntcompThreehundredRealM+\SemmlASemmlSyntcompThreehundredRealK/\SemmlASemmlSyntcompThreehundredRealL]}
\newcommand{\SemmlASemmlSyntcompThreehundredUnrealT}{1.11}
\newcommand{\SemmlASemmlSyntcompThreehundredUnrealM}{14}
\newcommand{\SemmlASemmlSyntcompThreehundredUnrealK}{8}
\newcommand{\SemmlASemmlSyntcompThreehundredUnrealL}{7}
\newcommand{\SemmlASemmlSyntcompThreehundredUnrealScore}{\SemmlASemmlSyntcompThreehundredUnrealT[\SemmlASemmlSyntcompThreehundredUnrealM+\SemmlASemmlSyntcompThreehundredUnrealK/\SemmlASemmlSyntcompThreehundredUnrealL]}
\newcommand{\StrixRealSyntheticThreehundred}{4}
\newcommand{\StrixUnrealSyntheticThreehundred}{10}
\newcommand{\SemmlARealSyntheticThreehundred}{23}
\newcommand{\SemmlAUnrealSyntheticThreehundred}{28}
\newcommand{\SemmlRealSyntheticThreehundred}{31}
\newcommand{\SemmlUnrealSyntheticThreehundred}{36}
\newcommand{\trivialSyntheticThreehundred}{16}
\newcommand{\nontrivialSyntheticThreehundred}{184}
\newcommand{\trivialStrixSemmlASyntheticThreehundred}{17}
\newcommand{\unknownStrixSemmlASyntheticThreehundred}{133}
\newcommand{\StrixSemmlASyntheticThreehundredAllT}{12.78}
\newcommand{\StrixSemmlASyntheticThreehundredAllM}{13}
\newcommand{\StrixSemmlASyntheticThreehundredAllK}{0}
\newcommand{\StrixSemmlASyntheticThreehundredAllL}{37}
\newcommand{\StrixSemmlASyntheticThreehundredAllScore}{\StrixSemmlASyntheticThreehundredAllT[\StrixSemmlASyntheticThreehundredAllM+\StrixSemmlASyntheticThreehundredAllK/\StrixSemmlASyntheticThreehundredAllL]}
\newcommand{\StrixSemmlASyntheticThreehundredRealT}{11.79}
\newcommand{\StrixSemmlASyntheticThreehundredRealM}{4}
\newcommand{\StrixSemmlASyntheticThreehundredRealK}{0}
\newcommand{\StrixSemmlASyntheticThreehundredRealL}{19}
\newcommand{\StrixSemmlASyntheticThreehundredRealScore}{\StrixSemmlASyntheticThreehundredRealT[\StrixSemmlASyntheticThreehundredRealM+\StrixSemmlASyntheticThreehundredRealK/\StrixSemmlASyntheticThreehundredRealL]}
\newcommand{\StrixSemmlASyntheticThreehundredUnrealT}{13.25}
\newcommand{\StrixSemmlASyntheticThreehundredUnrealM}{9}
\newcommand{\StrixSemmlASyntheticThreehundredUnrealK}{0}
\newcommand{\StrixSemmlASyntheticThreehundredUnrealL}{18}
\newcommand{\StrixSemmlASyntheticThreehundredUnrealScore}{\StrixSemmlASyntheticThreehundredUnrealT[\StrixSemmlASyntheticThreehundredUnrealM+\StrixSemmlASyntheticThreehundredUnrealK/\StrixSemmlASyntheticThreehundredUnrealL]}
\newcommand{\trivialStrixSemmlSyntheticThreehundred}{16}
\newcommand{\unknownStrixSemmlSyntheticThreehundred}{117}
\newcommand{\StrixSemmlSyntheticThreehundredAllT}{13.44}
\newcommand{\StrixSemmlSyntheticThreehundredAllM}{14}
\newcommand{\StrixSemmlSyntheticThreehundredAllK}{0}
\newcommand{\StrixSemmlSyntheticThreehundredAllL}{53}
\newcommand{\StrixSemmlSyntheticThreehundredAllScore}{\StrixSemmlSyntheticThreehundredAllT[\StrixSemmlSyntheticThreehundredAllM+\StrixSemmlSyntheticThreehundredAllK/\StrixSemmlSyntheticThreehundredAllL]}
\newcommand{\StrixSemmlSyntheticThreehundredRealT}{13.13}
\newcommand{\StrixSemmlSyntheticThreehundredRealM}{4}
\newcommand{\StrixSemmlSyntheticThreehundredRealK}{0}
\newcommand{\StrixSemmlSyntheticThreehundredRealL}{27}
\newcommand{\StrixSemmlSyntheticThreehundredRealScore}{\StrixSemmlSyntheticThreehundredRealT[\StrixSemmlSyntheticThreehundredRealM+\StrixSemmlSyntheticThreehundredRealK/\StrixSemmlSyntheticThreehundredRealL]}
\newcommand{\StrixSemmlSyntheticThreehundredUnrealT}{13.56}
\newcommand{\StrixSemmlSyntheticThreehundredUnrealM}{10}
\newcommand{\StrixSemmlSyntheticThreehundredUnrealK}{0}
\newcommand{\StrixSemmlSyntheticThreehundredUnrealL}{26}
\newcommand{\StrixSemmlSyntheticThreehundredUnrealScore}{\StrixSemmlSyntheticThreehundredUnrealT[\StrixSemmlSyntheticThreehundredUnrealM+\StrixSemmlSyntheticThreehundredUnrealK/\StrixSemmlSyntheticThreehundredUnrealL]}
\newcommand{\trivialSemmlASemmlSyntheticThreehundred}{45}
\newcommand{\unknownSemmlASemmlSyntheticThreehundred}{113}
\newcommand{\SemmlASemmlSyntheticThreehundredAllT}{2.24}
\newcommand{\SemmlASemmlSyntheticThreehundredAllM}{18}
\newcommand{\SemmlASemmlSyntheticThreehundredAllK}{4}
\newcommand{\SemmlASemmlSyntheticThreehundredAllL}{20}
\newcommand{\SemmlASemmlSyntheticThreehundredAllScore}{\SemmlASemmlSyntheticThreehundredAllT[\SemmlASemmlSyntheticThreehundredAllM+\SemmlASemmlSyntheticThreehundredAllK/\SemmlASemmlSyntheticThreehundredAllL]}
\newcommand{\SemmlASemmlSyntheticThreehundredRealT}{3.47}
\newcommand{\SemmlASemmlSyntheticThreehundredRealM}{8}
\newcommand{\SemmlASemmlSyntheticThreehundredRealK}{2}
\newcommand{\SemmlASemmlSyntheticThreehundredRealL}{10}
\newcommand{\SemmlASemmlSyntheticThreehundredRealScore}{\SemmlASemmlSyntheticThreehundredRealT[\SemmlASemmlSyntheticThreehundredRealM+\SemmlASemmlSyntheticThreehundredRealK/\SemmlASemmlSyntheticThreehundredRealL]}
\newcommand{\SemmlASemmlSyntheticThreehundredUnrealT}{1.57}
\newcommand{\SemmlASemmlSyntheticThreehundredUnrealM}{10}
\newcommand{\SemmlASemmlSyntheticThreehundredUnrealK}{2}
\newcommand{\SemmlASemmlSyntheticThreehundredUnrealL}{10}
\newcommand{\SemmlASemmlSyntheticThreehundredUnrealScore}{\SemmlASemmlSyntheticThreehundredUnrealT[\SemmlASemmlSyntheticThreehundredUnrealM+\SemmlASemmlSyntheticThreehundredUnrealK/\SemmlASemmlSyntheticThreehundredUnrealL]}
\newcommand{\StrixRealSyntcomptfThreehundred}{39}
\newcommand{\StrixUnrealSyntcomptfThreehundred}{27}
\newcommand{\SemmlARealSyntcomptfThreehundred}{49}
\newcommand{\SemmlAUnrealSyntcomptfThreehundred}{38}
\newcommand{\SemmlRealSyntcomptfThreehundred}{51}
\newcommand{\SemmlUnrealSyntcomptfThreehundred}{37}
\newcommand{\trivialSyntcomptfThreehundred}{912}
\newcommand{\nontrivialSyntcomptfThreehundred}{199}
\newcommand{\trivialStrixSemmlASyntcomptfThreehundred}{912}
\newcommand{\unknownStrixSemmlASyntcomptfThreehundred}{79}
\newcommand{\StrixSemmlASyntcomptfThreehundredAllT}{3.26}
\newcommand{\StrixSemmlASyntcomptfThreehundredAllM}{33}
\newcommand{\StrixSemmlASyntcomptfThreehundredAllK}{33}
\newcommand{\StrixSemmlASyntcomptfThreehundredAllL}{54}
\newcommand{\StrixSemmlASyntcomptfThreehundredAllScore}{\StrixSemmlASyntcomptfThreehundredAllT[\StrixSemmlASyntcomptfThreehundredAllM+\StrixSemmlASyntcomptfThreehundredAllK/\StrixSemmlASyntcomptfThreehundredAllL]}
\newcommand{\StrixSemmlASyntcomptfThreehundredRealT}{3.8}
\newcommand{\StrixSemmlASyntcomptfThreehundredRealM}{25}
\newcommand{\StrixSemmlASyntcomptfThreehundredRealK}{14}
\newcommand{\StrixSemmlASyntcomptfThreehundredRealL}{24}
\newcommand{\StrixSemmlASyntcomptfThreehundredRealScore}{\StrixSemmlASyntcomptfThreehundredRealT[\StrixSemmlASyntcomptfThreehundredRealM+\StrixSemmlASyntcomptfThreehundredRealK/\StrixSemmlASyntcomptfThreehundredRealL]}
\newcommand{\StrixSemmlASyntcomptfThreehundredUnrealT}{2.03}
\newcommand{\StrixSemmlASyntcomptfThreehundredUnrealM}{8}
\newcommand{\StrixSemmlASyntcomptfThreehundredUnrealK}{19}
\newcommand{\StrixSemmlASyntcomptfThreehundredUnrealL}{30}
\newcommand{\StrixSemmlASyntcomptfThreehundredUnrealScore}{\StrixSemmlASyntcomptfThreehundredUnrealT[\StrixSemmlASyntcomptfThreehundredUnrealM+\StrixSemmlASyntcomptfThreehundredUnrealK/\StrixSemmlASyntcomptfThreehundredUnrealL]}
\newcommand{\trivialStrixSemmlSyntcomptfThreehundred}{921}
\newcommand{\unknownStrixSemmlSyntcomptfThreehundred}{84}
\newcommand{\StrixSemmlSyntcomptfThreehundredAllT}{3.58}
\newcommand{\StrixSemmlSyntcomptfThreehundredAllM}{30}
\newcommand{\StrixSemmlSyntcomptfThreehundredAllK}{27}
\newcommand{\StrixSemmlSyntcomptfThreehundredAllL}{49}
\newcommand{\StrixSemmlSyntcomptfThreehundredAllScore}{\StrixSemmlSyntcomptfThreehundredAllT[\StrixSemmlSyntcomptfThreehundredAllM+\StrixSemmlSyntcomptfThreehundredAllK/\StrixSemmlSyntcomptfThreehundredAllL]}
\newcommand{\StrixSemmlSyntcomptfThreehundredRealT}{3.14}
\newcommand{\StrixSemmlSyntcomptfThreehundredRealM}{24}
\newcommand{\StrixSemmlSyntcomptfThreehundredRealK}{12}
\newcommand{\StrixSemmlSyntcomptfThreehundredRealL}{24}
\newcommand{\StrixSemmlSyntcomptfThreehundredRealScore}{\StrixSemmlSyntcomptfThreehundredRealT[\StrixSemmlSyntcomptfThreehundredRealM+\StrixSemmlSyntcomptfThreehundredRealK/\StrixSemmlSyntcomptfThreehundredRealL]}
\newcommand{\StrixSemmlSyntcomptfThreehundredUnrealT}{6.06}
\newcommand{\StrixSemmlSyntcomptfThreehundredUnrealM}{6}
\newcommand{\StrixSemmlSyntcomptfThreehundredUnrealK}{15}
\newcommand{\StrixSemmlSyntcomptfThreehundredUnrealL}{25}
\newcommand{\StrixSemmlSyntcomptfThreehundredUnrealScore}{\StrixSemmlSyntcomptfThreehundredUnrealT[\StrixSemmlSyntcomptfThreehundredUnrealM+\StrixSemmlSyntcomptfThreehundredUnrealK/\StrixSemmlSyntcomptfThreehundredUnrealL]}
\newcommand{\trivialSemmlASemmlSyntcomptfThreehundred}{951}
\newcommand{\unknownSemmlASemmlSyntcomptfThreehundred}{102}
\newcommand{\SemmlASemmlSyntcomptfThreehundredAllT}{0.97}
\newcommand{\SemmlASemmlSyntcomptfThreehundredAllM}{39}
\newcommand{\SemmlASemmlSyntcomptfThreehundredAllK}{9}
\newcommand{\SemmlASemmlSyntcomptfThreehundredAllL}{10}
\newcommand{\SemmlASemmlSyntcomptfThreehundredAllScore}{\SemmlASemmlSyntcomptfThreehundredAllT[\SemmlASemmlSyntcomptfThreehundredAllM+\SemmlASemmlSyntcomptfThreehundredAllK/\SemmlASemmlSyntcomptfThreehundredAllL]}
\newcommand{\SemmlASemmlSyntcomptfThreehundredRealT}{0.9}
\newcommand{\SemmlASemmlSyntcomptfThreehundredRealM}{25}
\newcommand{\SemmlASemmlSyntcomptfThreehundredRealK}{1}
\newcommand{\SemmlASemmlSyntcomptfThreehundredRealL}{3}
\newcommand{\SemmlASemmlSyntcomptfThreehundredRealScore}{\SemmlASemmlSyntcomptfThreehundredRealT[\SemmlASemmlSyntcomptfThreehundredRealM+\SemmlASemmlSyntcomptfThreehundredRealK/\SemmlASemmlSyntcomptfThreehundredRealL]}
\newcommand{\SemmlASemmlSyntcomptfThreehundredUnrealT}{1.11}
\newcommand{\SemmlASemmlSyntcomptfThreehundredUnrealM}{14}
\newcommand{\SemmlASemmlSyntcomptfThreehundredUnrealK}{8}
\newcommand{\SemmlASemmlSyntcomptfThreehundredUnrealL}{7}
\newcommand{\SemmlASemmlSyntcomptfThreehundredUnrealScore}{\SemmlASemmlSyntcomptfThreehundredUnrealT[\SemmlASemmlSyntcomptfThreehundredUnrealM+\SemmlASemmlSyntcomptfThreehundredUnrealK/\SemmlASemmlSyntcomptfThreehundredUnrealL]}

==> preamble/0_macros.tex <==
% == LATEX
%\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

%\newcolumntype{L}{X}
%\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
%\newcolumntype{C}{>{\centering\arraybackslash}X}

\RequirePackage{amsmath}
\RequirePackage{amssymb}

% == SYMBOLS

\RequirePackage{marvosym}
\providecommand{\contradiction}{\Lightning}

% == BASIC OPERATORS

\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\pospart}{\lgroup}{\rgroup^+}
\DeclarePairedDelimiter{\negpart}{\lgroup}{\rgroup^-}
\DeclarePairedDelimiterX{\inner}[2]{\lange}{\rangle}{#1, #2}
\DeclarePairedDelimiter{\cardinality}{\lvert}{\rvert}
\DeclarePairedDelimiter{\set}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\tuple}{(}{)}
\DeclarePairedDelimiter{\listt}{[}{]}


% == SETS OPERATORS

\newcommand{\setcomplement}[1]{{#1}^c}
\newcommand{\powerset}[1]{\mathcal{P}(#1)}

\newcommand{\unionSym}{\cup}
\newcommand{\unionBin}{\mathbin{\unionSym}}
\newcommand{\strictunionSym}{\dot{\unionSym}}
\newcommand{\strictunionBin}{\mathbin{\dot{\unionSym}}}
\newcommand{\intersectionSym}{\cap}
\newcommand{\intersectionBin}{\mathbin{\intersectionSym}}
\newcommand{\UnionSym}{\bigcup}
\newcommand{\UnionBin}{\mathbin{\UnionSym}}
\newcommand{\strictUnionSym}{\dot{\UnionSym}}
\newcommand{\strictUnionBin}{\mathbin{\strictUnionSym}}
\newcommand{\IntersectionSym}{\bigcap}
\newcommand{\IntersectionBin}{\mathbin{\IntersectionSym}}

\newcommand{\union}{\unionBin}
\newcommand{\strictunion}{\strictunionBin}
\newcommand{\intersection}{\intersectionBin}
\newcommand{\Union}{\UnionSym}
\newcommand{\strictUnion}{\strictUnionSym}
\newcommand{\Intersection}{\IntersectionSym}


% == BASIC SETS

\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Rationals}{\mathbb{Q}}
\newcommand{\Reals}{\mathbb{R}}


% == OPERATORS

\newcommand{\gradient}{\nabla}
\newcommand{\laplacian}{\Delta}
\newcommand{\diff}{\partial}
\newcommand{\boundary}{\partial}
\DeclareMathOperator{\divergence}{div}
\DeclareMathOperator{\distance}{dist}
\DeclareMathOperator{\esssup}{ess sup}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\capacity}{cap}
\DeclareMathOperator{\signum}{signum}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\const}{const}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator*{\argmax}{arg\, max}
\DeclareMathOperator*{\argmin}{arg\, min}

\newcommand{\qee}{\hfill$\triangle$} % quod erat exemplandum

% == LOGIC

% lor, land, lnot etc already defined
\newcommand{\lOr}{\bigvee}
\newcommand{\lAnd}{\bigwedge}
\newcommand{\lfalse}{\texttt{ff}}
\newcommand{\ltrue}{\texttt{tt}}

\DeclareMathOperator{\ExistsOp}{\exists}
\DeclareMathOperator{\ForallOp}{\forall}

\newcommand{\LTL}{\operatorname{LTL}}
\newcommand{\CTL}{\operatorname{CTL}}
\newcommand{\PCTL}{\operatorname{pCTL}}

\newcommand{\ltlNext}{\operatorname{\mathbf{X}}}
\newcommand{\ltlFinally}{\operatorname{\mathbf{F}}}
\newcommand{\ltlGlobally}{\operatorname{\mathbf{G}}}
\newcommand{\ltlUntil}{\mathbin{\mathbf{U}}}
\newcommand{\ltlWuntil}{\mathbin{\mathbf{W}}}
\newcommand{\ltlRelease}{\mathbin{\mathbf{R}}}
\newcommand{\ltlSrelease}{\mathbin{\mathbf{M}}}
\newcommand{\ltlLanguage}[1]{\mathcal{L}(#1)}
\newcommand{\true}{\texttt{tt}}
\newcommand{\false}{\texttt{ff}}
\newcommand{\trueness}{t}

\newcommand{\Alphabet}{\Sigma}
\newcommand{\AP}{\mathsf{AP}}

\DeclareMathOperator{\subformulas}{sub}
\DeclareMathOperator{\topformulas}{top}

\DeclareMathOperator{\satisfying}{sat}

% == COMPLEXITY

\newcommand{\NP}{\mathbf{NP}}
\newcommand{\coNP}{\mathbf{coNP}}
\newcommand{\NEXP}{\mathbf{NEXP}}
\newcommand{\PSPACE}{\mathbf{PSPACE}}

% == GAMES

\newcommand{\G}{\mathcal{G}}
\newcommand{\Vertices}{V}
\newcommand{\Edges}{E}
\newcommand{\VertexPlayer}{P}
\newcommand{\EdgesSys}{E_\sys}
\newcommand{\EdgesEnv}{E_\env}
\newcommand{\initialvertex}{v_0}
\newcommand{\play}{\rho}
\newcommand{\Plays}{\mathfrak{P}}
\newcommand{\player}{p}
\newcommand{\strategy}{\sigma}
\newcommand{\priorities}{\mathfrak{p}}

\newcommand{\sys}{\mathcal{S}}
\newcommand{\env}{\mathcal{E}}
\newcommand{\VerticesSys}{\Vertices_\sys}
\newcommand{\VerticesEnv}{\Vertices_\env}

\newcommand{\GExt}{\mathsf{Ext}}
% == OTHER

\DeclareMathOperator{\obligationSetFormula}{\emph{osf}}
\DeclareMathOperator{\someAssignment}{\mathcal{A}}

\newcommand{\smallenv}{\mathsf{ENV}}%{\text{\small\textsc{ENV}}}
\newcommand{\smallsys}{\mathsf{SYS}}%{\text{\small\textsc{SYS}}}

%\newcommand{\para}[1]{{\smallskip\noindent\textbf{#1}}}
\newcommand{\para}[1]{\paragraph{#1}}

\input{data/table_commands.tex}

\newcommand{\SemML}{\textsc{SemML}}
\newcommand{\Strix}{\textsc{Strix}}
\newcommand{\Owl}{\textsc{Owl}}
\newcommand{\SemMLs}{\SemML\textsubscript{S}}
\newcommand{\SemMLa}{%
\def\ULthickness{1pt}%
\textsc{Sem\sout{ML}}%
}
\newcommand{\Syntcomp}{\textsc{SYNTCOMP}}
\newcommand{\Neurosynt}{\textsc{NeuroSynt}}

\newcommand{\Sum} [2] {\the\numexpr #1 + #2 \relax}
\newcommand{\Diff} [2] {\the\numexpr #1 - #2 \relax}

